A Spectral Approach to Item Response Theory

The Rasch model is one of the most fundamental models in \emph{item response theory} and has wide-ranging applications from education testing to recommendation systems. In a universe with $n$ users and $m$ items, the Rasch model assumes that the binary response $X_{li} \in \{0,1\}$ of a user $l$ with parameter $\theta^*_l$ to an item $i$ with parameter $\beta^*_i$ (e.g., a user likes a movie, a student correctly solves a problem) is distributed as $\Pr(X_{li}=1) = 1/(1 + \exp{-(\theta^*_l - \beta^*_i)})$. In this paper, we propose a \emph{new item estimation} algorithm for this celebrated model (i.e., to estimate $\beta^*$). The core of our algorithm is the computation of the stationary distribution of a Markov chain defined on an item-item graph. We complement our algorithmic contributions with finite-sample error guarantees, the first of their kind in the literature, showing that our algorithm is consistent and enjoys favorable optimality properties. We discuss practical modifications to accelerate and robustify the algorithm that practitioners can adopt. Experiments on synthetic and real-life datasets, ranging from small education testing datasets to large recommendation systems datasets show that our algorithm is scalable, accurate, and competitive with the most commonly used methods in the literature.

==> analysis/analysis.tex <==

Inspired by the literature on Spectral Ranking algorithms under the BTL model \cite{negahban2017rank,chen2019spectral,agarwal2018accelerated}, we seek to construct a Markov Chain such that the resulting stationary distribution coincides (or can be easily transformed into) the parameters of the Rasch model that we are interested in estimating. It's notable that under the BTL model, the idealized Markov Chain is reversible. This allows for tight perturbation bound on the stationary distribution (cf. Lemma 2 of \cite{negahban2017rank}, Theorem 8 of \cite{chen2019spectral}, Theorem 2 of \cite{agarwal2018accelerated}). This property is highly specialized to the distribution assumptions of the BTL model. Under the Rasch model, it is possible to construct such a Markov Chain. In fact, there can be more than one way to construct a desired Markov Chain.

~\\
Define
% \begin{equation}\label{eqn:normalized-bij}
% \bar B^*_{ij} = \frac{1}{\lvert \Ss_{ij}\rvert} \cdot \sum_{l\in \Ss_{ij}} \E[X_{li}(1-X_{lj})] =  \frac{1}{\lvert \Ss_{ij}\rvert} \cdot \sum_{l\in \Ss_{ij}} \frac{w^*_l}{w^*_l + z^*_i} \cdot \frac{z_j^*}{w^*_l + z_j^*} 
% \end{equation}
% where $\Ss_{ij}$ is the set of students assigned problems $i, j$. This is a random variable. 
% Alternatively, define
\begin{equation}\label{eqn:unnormalized-bij}
D^*_{ij} = \sum_{l\in [n]} \E[A_{li} A_{lj} X_{pi}(1-X_{lj})] =  \sum_{l\in[n]} p^2\frac{w^*_l}{w^*_l + z^*_i} \cdot \frac{z_j^*}{w^*_l + z_j^*} 
\end{equation}
where $A_{li}$ is the indicator random variable whether student $l$ is assigned problem $i$.

~\\
Consider a Markov Chain defined entrywise as follows:
\begin{equation}\label{eqn:markov-chain-def}
P^*_{ij} = \begin{cases} \frac{1}{d_i} D^*_{ij} &\text{ if $i \neq j$}\\
1 - \sum_{k\neq i} \frac{1}{d_i} D^*_{ik} &\text{ if $i = j$}
\end{cases}
\end{equation}
where $d_i$ is a problem specific normalization factor to ensure that we have a valid transition matrix. We could have $d_1=\ldots=d_m = d$ for some sufficiently large $d$. We also assume that the graph underlying the Markov Chain is connected, this is to ensure that the stationary distribution is unique. We will now show that the above Markov Chain is reversible and that the parameters $z^*$ can be recovered from its stationary distribution.

\begin{theorem}\label{thm:reversible-mc} The Markov Chain constructed per \ref{eqn:markov-chain-def} is reversible. That is for every pair of state $i \neq j$ 
$$ \pi^*_i P^*_{ij} = \pi^*_j P^*_{ji} $$
where $z_i^* = \frac{1}{d_i} \cdot \pi^*_i$.
\end{theorem}

\begin{proof} We have
\begin{equation*}
\begin{aligned}
\pi_i^* P^*_{ij} &= d_i z_i^*  \frac{1}{d_i} D^*_{ij} \\
&= z_i^*\sum_{l\in [m]}p^2 \frac{w^*_l}{w^*_l + z^*_i} \cdot \frac{z_j^*}{w^*_l + z_j^*} \\
&= z_j^* \sum_{l\in [m]}p^2 \frac{w^*_l}{w^*_l + z^*_j} \cdot \frac{z_i^*}{w^*_l + z_i^*} \\
&= d_jz_j^*  \frac{1}{d_j} D_{ji}^*\\
&= \pi_j^* P^*_{ji}
\end{aligned}
\end{equation*}
This completes the proof.
\end{proof}

Reversibility and connectedness of the underlying graph ensure that the stationary distribution of the Markov Chain is unique. Note that the above analysis pertains to the idealized Markov Chain $P^*$. Let us now define the empirical Markov Chain constructed from observed student-problem performance data.


Consider the problem setup in section \ref{sect:problem-setup}. Additionally, assume that for each student $l$, each problem $i$ is independently given to that student with probability $p$. Let $A_{li}$ denote the indicator random variable whether student $l$ is given problem $i$. Note that we assume a fixed dynamic range $\kappa = z^*_{\max} - z_{\min}^*$.
Recall the construction of the Markov Chain per equations \ref{eqn:Dij} and \ref{eqn:emp-markov-chain-def}. Define $B_{ij} = \sum_{l}A_{li}A_{lj}$ and the following events:
$$ \A = \{ \frac{np^2}{2} \leq B_{ij} \leq \frac{3np^2}{2} \,\forall i\neq j\in [m] \} $$
$$ \A^+ = \A \cap \{ \frac{mp}{2} \leq A_{l}^\top \mb 1 \leq \frac{3mp}{2} \,\forall l \in [n] \}$$

\begin{lemma} Consider the sampling scheme above,
$$ \Pr(\A) \geq 1 - \frac{1}{m^C} $$
so long as $np^2 \gtrsim \log m$ by a sufficiently large constant.
\end{lemma}

\begin{lemma} Consider the sampling scheme above,
$$ \Pr(\A^+) \geq 1 - \frac{1}{m^C} - \frac{1}{n^C} $$
so long as $np^2 \gtrsim \log m$ and $mp \gtrsim \log n$ by a sufficiently large constant.
\end{lemma}

One consequence of the assumption $np^2 \gtrsim \log m$ is that $\sum_{l=1}^n A_{li} \leq \frac{3np}{2}$ with high probability for all $i \in [m]$.
We first restate some useful results which provide bounds on the total variation distance distance and the $\ell_2$ error of the stationary distribution of a Markov Chain $P$ from a \emph{reference reversible Markov Chain} $P^*$. In all of the following lemmas, $\mu^*(P)$ is the spectral gap of the reference Markov Chain.


~\\
\textbf{a. Total variation perturbation bound for reversible Markov Chains}
\begin{lemma}\label{lem:total-variation-bound-mc} (Theorem 2 of \citet{agarwal2018accelerated}, originally due to \citet{mitrophanov2005sensitivity}) Consider two discrete time Markov Chain $P$ and $P^*$ with finite state space and stationary distribution $\pi$ and $\pi^*$, respectively. If there exists a positive constants $R > 1$ and $\rho < 1$ such that:
$$ \lVert P^t(x, \cdot) - \pi^* \rVert_{TV} \leq R\rho^t, t = 1, 2,\ldots $$
then we have:
$$ \lVert \pi - \pi^* \rVert_{TV} \lesssim \frac{1}{\mu(P^*)} \lVert P - P^* \rVert_{\infty} $$
\end{lemma}

~\\
\textbf{b. $\ell_2$ perturbation bound for reversible Markov Chains}
\begin{lemma} (Lemma 2 of \citet{negahban2017rank}) Consider the setting of lemma \ref{lem:total-variation-bound-mc}, then:
$$ \frac{\lVert \pi - \pi^* \rVert}{\lVert \pi^*\rVert} \lesssim \frac{1}{\mu({P^*})} \lVert P - P^* \rVert_{2} $$
\end{lemma}

\begin{lemma} (Lemma 8 of \citet{chen2019spectral}) Consider the setting of lemma \ref{lem:total-variation-bound-mc}, then:
$$ \lVert \pi - \pi^* \rVert_{\pi^*} \leq \frac{\lVert {\pi^*}^\top(P^* - P)\rVert_{\pi^*}  }{\mu(P^*) - \lVert P - P^* \rVert_{\pi^*} } $$
where $\mu(P^*)$ is the spectral gap of $P^*$.
\end{lemma}

\subsection{Bounding the spectral gap $\mu(P^*)$}

\begin{theorem} Suppose that $np^2\gtrsim \log m$, then
$$\mu(P^*) \gtrsim \frac{nmp^2}{d} $$
\end{theorem}

\begin{proof} Here we follow similar steps to the proof of Lemma 4 in \citet{negahban2017rank}. The goal is to construct a reversible Markov Chain whose spectral gap is easier to analyze and use a comparison Lemma 6 of \citet{negahban2017rank} (originally due to \citet{diaconis1993comparison}) to obtain a lower bound on the spectral gap of $P^*$. To this end, consider the following Markov Chain:
$$ \tilde P_{ij} = \frac{B_{ij}}{d}\quad \forall i\neq j $$
and
$$\tilde P_{ii} = 1 - \sum_{j\neq i} \tilde P_{ij} $$
% Following similar argument as in the proof of Lemma 4 in \citet{negahban2017rank}, we have:
% $$ \mu(P^*) \gtrsim \mu(\tilde P) $$
% It suffices to lower bound $\mu(\tilde P) =  1 - \max_{u: \lVert u \rVert_1, u \indep \mb 1} u^\top \tilde Pu = \frac{1}{d} \min_{u: \lVert u \rVert_1, u \indep \mb 1} u^\top \tilde L u $ where $\tilde L = \tilde D - \tilde A$ is the Laplacian of the weighted graph corresponding to $B$ (without the normalization factor $d$). Conditioned on event $\A$, we have:
% $$ $$
Define the Laplacian $L = D- B$ where $D$ is a diagonal matrix with $D_{ii} = \sum_{j\neq i} B_{ij}$. Then one can verify that:
$$ \tilde P = I - \frac{L}{d} $$
As such:
$$ \mu(\tilde P) = \mu(I - \frac{L}{d}) = \frac{1}{d}\lambda_{\min, \indep}(L) $$
Following similar argument as in the proof of Lemma A.3 in \citet{gao2021uncertainty}, we have:
$$ \lambda_{\min,\indep}(L) \gtrsim mnp^2 $$
This completes the proof.
\end{proof}

\subsection{Bounding the error term $\lVert P - P^* \rVert_2$}

\begin{theorem} Suppose that $np^2\gtrsim \log m$
$$\lVert P - P^* \rVert_2 \lesssim \frac{\epsilon nmp^2}{d} $$
for some small constant $\epsilon$.
\end{theorem}


\begin{proof}
As shown previously, so long as $np^2 \gtrsim \log m$, then $\lvert P_{ij} - P^*_{ij}\rvert \lesssim \frac{np^2\epsilon}{d}$ with high probability. We have:
\begin{equation*}
\begin{aligned}
\lVert P - P^* \rVert_2 &\leq \lVert \diag(P) I - \diag(P^*) I\rVert_{op} + \lVert [P - P^*]_{i\neq j}\rVert_{op} \\
&\leq \max_{i} \lvert P_{ii} - P_{ii} \rvert + \max_{u, v} \sum_{i\neq j} u_i (P_{ij} - P_{ij}^*)v_j\\
&\leq \max_{i} \lvert \sum_{j\neq i} P_{ij}-P_{ij}^* \rvert + \max_{i\neq j} \lvert P_{ij}-P^*_{ij}\rvert \cdot \sum_{i\neq j} \lvert u_i\rvert \lvert v_j\rvert\\
&\leq 2 m \cdot \max_{i\neq j} \lvert P_{ij} - P_{ij}^* \rvert \\
&\lesssim \frac{\epsilon mnp^2}{d}
\end{aligned}
\end{equation*}
This completes the proof.
\end{proof}

\subsection{Bounding the projected error term $\lVert {\pi^*}^\top (P - P^*)\rVert_2 $}
To make progress we follow a simlar argument as in the proof of Lemma 8.4 in \citet{gao2021uncertainty} in turning the norm term into a linear term. Specifically, we have:
\begin{equation*}
\begin{aligned}
\lVert {\pi^*}^\top (P - P^*)\rVert_2 &= \sqrt{\sum_{i=1}^n\bigg(\sum_{j=1}^n \pi_j^*(P_{ji}-P_{ji}^*) \bigg)}\\
&= \sqrt{\sum_{i=1}^n\bigg(\sum_{j\neq i} \pi_j^*(P_{ji}-P_{ji}^*) + \pi_i^*(P_{ii}-P_{ii}^*) \bigg)}\\
&= \sqrt{\sum_{i=1}^n\bigg(\sum_{j\neq i} \pi_j^*(P_{ji}-P_{ji}^*) + \pi_i^*(\sum_{j\neq i} P^*_{ij}-P_{ij}) \bigg)}\\
&=  \sqrt{\sum_{i=1}^n\bigg(\sum_{j\neq i} \pi_j^*(P_{ji}-P_{ji}^*) + \pi_i^* (P^*_{ij}-P_{ij}) \bigg)}\\
&\leq 2 \max_{v\in \mathcal{V}} \sum_{i=1}^n v_i \bigg(\sum_{j\neq i} \pi_j^*(P_{ji}-P_{ji}^*) + \pi_i^*(P_{ij}^* - P_{ij})  \bigg)
\end{aligned}
\end{equation*}
where $\mathcal{V}$ is a $\frac{1}{2}$-covering of the unit norm ball. Now noting that $\pi_i^* = \bar z^*_i$ where $\bar z_i^* = \frac{z_i^*}{\sum_{j} z_j^*}$ is the normalized version of the test parameters. 


\subsubsection{Bounded difference method}
We first show that the linear term can be rewritten as follows:
\begin{equation*}
\begin{aligned}
&d\sum_{i=1}^m v_i \bigg( \sum_{j\neq i} \pi_j^* (P_{ji} - P_{ji}^*) + \pi_i^*(P_{ij}^* - P_{ij}) \bigg)\\
&= \sum_{l=1}^n \sum_{i=1}^m \sum_{j\neq i} \bigg( (v_i - v_j)\pi_j^*A_{li}A_{lj} \big[(X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})]\big]\bigg)
\end{aligned}
\end{equation*}
Note that (ignoring the expectation terms) this sum is a function $f$ of $m\times n$ independent random variables $\{X_{li}\}$. Let $X$ and $X'$ be identical copies except for $X_{li}\neq X'_{li}$.
\begin{equation*} 
\begin{aligned}
 f(X) - f(X') &= \sum_{j\neq i} A_{li}A_{lj}(v_i - v_j) [X_{lj}(\pi^*_i - \pi_j^*) - \pi_i^*] \\
& \underset{\text{Cauchy-Schwarz}}{\leq} \frac{\kappa}{\sqrt m} \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj}(v_i - v_j)^2}
\end{aligned}
\end{equation*}
Applying Hoeffding's inequality now gives us:
\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n \sum_{i=1}^m \sum_{j\neq i} \bigg( (v_i - v_j)\pi_j^*A_{li}A_{lj} \big[(X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})]\big]\bigg)\\
&\lesssim  \frac{\kappa}{\sqrt m} \cdot \underbrace{\sqrt{\sum_{i\neq j}(v_i - v_j)^2 B_{ij}}}_{\lesssim \sqrt{mnp^2}}\\
&\lesssim \kappa \sqrt{np^2}
\end{aligned}
\end{equation*}
Applying union bound over all $v\in \mathcal{V}$ gives us:
$$ \lVert {\pi^*}^\top (P -P^*)\rVert_2 \lesssim \kappa\sqrt{mnp^2} $$


\subsubsection{Slightly tighter bound when $m$ is allowed to grow}

Note that one of the key step in the bounded difference analysis above is the Cauchy-Schwarz inequality. Conditioned on event $\A^+$ (same assumptions as $\A$ and $mp \gtrsim \log n$), we have slightly better bound.

\begin{equation*}
\begin{aligned}
 f(X) - f(X') &= \sum_{j\neq i} A_{li}A_{lj}(v_i - v_j) [X_{lj}(\pi^*_i - \pi_j^*) - \pi_i^*] \\
 &= \sum_{j\neq i} A_{lj}\cdot A_{li}A_{lj}(v_i - v_j) [\underbrace{X_{lj}(\pi^*_i - \pi_j^*) - \pi_i^*}_{\lesssim \frac{\kappa}{m}}] \\
& \underset{\text{Cauchy-Schwarz}}{\lesssim} \sqrt{\underbrace{\sum_{j\neq i} A_{lj}}_{\lesssim mp} } \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj}(v_i - v_j)^2} \cdot \frac{\kappa}{m}\\
&\lesssim \sqrt{mp}  \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj}(v_i - v_j)^2} \cdot \frac{\kappa}{m}\\
&\asymp \frac{\kappa\sqrt p}{\sqrt m} \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj}(v_i - v_j)^2} 
\end{aligned}
\end{equation*}

The rest of the analysis proceeds in the same way, giving us:
$$ \lVert {\pi^*}^\top (P- P^*)\rVert_2 \lesssim \kappa \sqrt{mnp^3} $$

% \subsubsection{Decomposition method}

\subsection{Summary}

~\\
\textbf{Error bound under small $m$ regime:} Using the bound from the bounded difference method with the previously shown bounds on the spectral gap and the transition matrix error term gives:
$$\lVert \pi^* - \pi\rVert_2 \lesssim \frac{\sqrt{mnp^2}}{mnp^2} \asymp \frac{1}{\sqrt{{mnp^2}}} $$

The error on the estimation of the difficulty parameters thus scales as:
$$ \lVert z - z^* \rVert_2 \lesssim \frac{\sqrt m}{\sqrt{np^2}} $$

~\\
\textbf{Error bound when $m$ is allowed to grow:} Conditioned on event $\A^+$ we obtain:
$$ \lVert {\pi^*}^\top (P - P^*)\rVert_2 \lesssim  \frac{\sqrt {mnp^3}}{d}  $$
The error on the estimation is:
$$ \lVert z - z^* \rVert_2 \lesssim \frac{\sqrt m}{\sqrt{np}} $$

~\\
The following table summarizes the results obtained thus far under two different regimes of $m$
\begin{centering}
\begin{table}[H]
\begin{tabular}{|l|l|l|}
\hline
                         & Constant $m$ regime & $m$ is allowed to grow \\ \hline
Assumptions              & $np^2 \gtrsim \log m$ & $np^2 \gtrsim \log m, mp \gtrsim \log n$ \\ \hline
Error bound on $\lVert z - z^* \rVert_2$ & $\sqrt{\frac{m}{np^2}}$ & $\sqrt{\frac{m}{np}}$  \\ \hline
Sufficient conditions for consistent estimation & $np^2 \gtrsim m\log m$ & $np \gtrsim \max\{m\log m, \sqrt n\sqrt{\log m}\}$, $mp \gtrsim \log n$ \\ \hline
\end{tabular}
\end{table}
\end{centering}


==> analysis/analysis_compact.tex <==


~\\
\begin{centering}
\begin{table}[H]
\begin{tabular}{|l|l|l|}
\hline
                         & Small $m$ regime & $m$ is allowed to grow \\ \hline
Assumptions              & $np^2 \gtrsim \log m$ & $np^2 \gtrsim \log m, mp \gtrsim \log n$ \\ \hline
Error bound on $\lVert z - z^* \rVert_2$ & $\sqrt{\frac{m}{np^2}}$ & $\sqrt{\frac{m}{np}}$  \\ \hline
\end{tabular}
\end{table}
\end{centering}


==> analysis/bounded_difference_approach.tex <==

\section{Proofs for the bounded difference method}
We first rewrite the linear term into a more manageable form:
\begin{equation*}
\begin{aligned}
&d\sum_{i=1}^m v_i \bigg( \sum_{j\neq i} \pi_j^* (P_{ji} - P_{ji}^*) + \pi_i^*(P_{ij}^* - P_{ij}) \bigg)\\
&=\sum_{i=1}^m v_i \bigg( \sum_{j\neq i} \pi_j^* \big[\sum_{l=1}^n A_{li}A_{lj}\big(X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})]\big) \big] \\
&\quad\quad- \sum_{j\neq i}\pi_i^* \big[\sum_{l=1}^n A_{li}A_{lj}\big(X_{li}(1-X_{lj}) - \E[X_{li}(1-X_{lj})]\big) \big] \bigg)\\
&=\sum_{l=1}^n\sum_{i=1}^m \bigg( \sum_{j\neq i} v_i \pi_j^*A_{li}A_{lj} \big[(X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})]\big]\big) \\
&-\sum_{l=1}^n\sum_{i=1}^m \bigg( \sum_{j\neq i} v_i \pi_i^*A_{li}A_{lj} \big[(X_{li}(1-X_{lj}) - \E[X_{li}(1-X_{lj})]\big]\big) \\
&= \sum_{l=1}^n \sum_{i=1}^m \sum_{j\neq i} \bigg( (v_i - v_j)\pi_j^*A_{li}A_{lj} \big[(X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})]\big]\bigg)
\end{aligned}
\end{equation*}

We will use the method of bounded difference to obtain a concentration inequality on the above sum. Note that this sum is essentially a function $f$ of $m\times n$ independent random variables $\{X_{li}\}$. Let $X$ and $X'$ be identical copies except for $X_{li}\neq X'_{li}$.
\begin{equation*} 
\begin{aligned}
\lvert f(X) - f(X')\rvert &= \lvert \sum_{j\neq i} A_{li}A_{lj}(v_i - v_j) [X_{lj}(\pi^*_i - \pi_j^*) - \pi_i^*] \rvert\\
% & \leq \sum_{j\neq i} \lvert A_{li}A_{lj}(v_i - v_j)  \underbrace{[X_{lj}(\pi^*_i - \pi_j^*) - \pi_i^*]}_{\leq \max\{\pi^*_i, \pi^*_j\}\lesssim \frac{\kappa}{m} }\rvert \\
% &\leq \sum_{j\neq i} \lvert A_{li}A_{lj} (v_i - v_j) \frac{\kappa}{m}\rvert \\
\end{aligned}
\end{equation*}
Using Cauchy-Schwarz, we have:
\begin{equation*} 
\begin{aligned}
% & \sum_{j\neq i} A_{li}A_{lj}(v_i - v_j) [X_{lj}(\pi^*_i - \pi_j^*) - \pi_i^*] \\
&\sum_{j\neq i}  A_{li}A_{lj}(v_i - v_j)  \underbrace{[X_{lj}(\pi^*_i - \pi_j^*) - \pi_i^*]}_{\leq \max\{\pi^*_i, \pi^*_j\} \lesssim \frac{\kappa}{m}}\\
% &\leq \sum_{j\neq i} \lvert A_{li}A_{lj} (v_i - v_j) \frac{\kappa}{m}\rvert \\
&\leq \frac{\kappa}{m} \cdot \sqrt m \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj}(v_i - v_j)^2} = \frac{\kappa}{\sqrt m} \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj}(v_i - v_j)^2}
\end{aligned}
\end{equation*}
Applying Hoeffding's inequality now gives us:
\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n \sum_{i=1}^m \sum_{j\neq i} \bigg( (v_i - v_j)\pi_j^*A_{li}A_{lj} \big[(X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})]\big]\bigg)\\
&\lesssim \sqrt{\sum_{l=1}^n\sum_{j=1}^m  \frac{\kappa^2}{m} \sum_{j\neq i} A_{li}A_{lj}(v_i - v_j)^2 }\\
&\asymp  \frac{\kappa}{\sqrt m} \cdot \underbrace{\sqrt{\sum_{i\neq j}(v_i - v_j)^2 B_{ij}}}_{\lesssim \sqrt{mnp^2}}\\
&\lesssim \kappa \sqrt{np^2}
\end{aligned}
\end{equation*}

We thus have
$$ \lVert {\pi^*}^\top (P -P^*)\rVert_2 \lesssim \kappa\sqrt{mnp^2} $$

==> analysis/decomposition_approach.tex <==
\textbf{Summary of the decomposition approach}

\begin{proposition}\label{prop:linear-decomp} Fixing an assignment $A$, we have:
\begin{equation*}
\begin{aligned}
&d\cdot\sum_{i=1}^m v_i \bigg(\sum_{j\neq i} \pi_j^*(P_{ji}-P_{ji}^*) + \pi_i^*(P_{ij}^* - P_{ij})  \bigg)\\
&=\sum_{l=1}^n \bigg( \sum_{i=1}^m v_i \sum_{j\neq i} A_{li}A_{lj} \bar z^*_j (X_{lj} - \E[X_{lj}]) \bigg) + \sum_{l=1}^n\bigg( \sum_{i=1}^m v_i\sum_{j\neq i} A_{li}A_{lj} \bar z^*_i (\E[X_{li}] - X_{li}) \bigg) \\
&+\sum_{l=1}^n\bigg(\sum_{i=1}^m v_i\sum_{j\neq i} A_{li}A_{lj} (\bar z^*_i-\bar z^*_j) (X_{li}X_{lj} - \E[X_{li}X_{lj}]) \bigg) \\
\end{aligned}
\end{equation*}
\end{proposition}


\begin{proposition}\label{prop:decomp-bound-first-linear-term} Conditioned on event $\A^+$, the first linear term is bounded by:
\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n \bigg( \sum_{i=1}^m v_i \sum_{j\neq i} A_{li}A_{lj} \bar z^*_j (X_{lj} - \E[X_{lj}]) \bigg)  \\
&= \sum_{l=1}^n \sum_{j=1}^m  (X_{lj} - \E[X_{lj}]) \cdot \bigg(A_{lj}\bar z^*_j v^\top A_l  \bigg) \lesssim \frac{\kappa}{m} \sqrt{mp} \sqrt{nmp^2}
\end{aligned}
\end{equation*}
\end{proposition}

\begin{proposition} \label{prop:decomp-bound-second-linear-term} Conditioned on event $\A^+$, the second linear term is bounded by:
\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n\bigg( \sum_{i=1}^m v_i\sum_{j\neq i} A_{li}A_{lj} \bar z^*_i (\E[X_{li}] - X_{li}) \bigg) \\
&= \sum_{l=1}^n\sum_{i=1}^m (\E[X_{li}] - X_{li}) \cdot  \bigg( v_i \bar z^*_i \sum_{j\neq i} A_{lj} \bigg) 
\lesssim \frac{\kappa}{m} \sqrt{mp}\sqrt{mnp^2}\\
\end{aligned}
\end{equation*}
\end{proposition}

~\\
The third quadratic term can be decomposed into 3 terms with two linear terms and a quadratic term.
\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n\bigg(\sum_{i=1}^m v_i\sum_{j\neq i} A_{li}A_{lj} (\bar z^*_i-\bar z^*_j) (X_{li}X_{lj} - \E[X_{li}X_{lj}]) \bigg)\\
&= \underbrace{ \sum_{l=1}^n(X_l-\E[X_l])^\top M^l (X_l-\E[X_l])}_{S_1} + \underbrace{ \sum_{l=1}^n(X_l - \E [X_l])^\top M^l \E[X_l]}_{S_2} + \underbrace{ \sum_{l=1}^n\E[X_l]^\top M^l (X_l - \E[X_l])}_{S_3} \\
\end{aligned}
\end{equation*}

\begin{proposition} Conditioned on $\A^+$,
$$ S_1 \lesssim \frac{\kappa}{m} \sqrt{mnp^2} $$ 
$$S_2 \lesssim \frac{\kappa}{m} \sqrt{mp}\sqrt{mnp^2}$$
$$S_3 \lesssim\frac{ \kappa}{m} \sqrt{mp}\sqrt{mnp^2}$$
Essentially,
$$ S_1 + S_2 + S_3 \lesssim  \frac{ \kappa}{m} \sqrt{mp}\sqrt{mnp^2} \asymp \sqrt{np^3} $$
\end{proposition}

~\\
\begin{remark}
On closer inspection, one can actually combine the first two linear terms 
\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n \bigg( \sum_{i=1}^m v_i \sum_{j\neq i} A_{li}A_{lj} \bar z^*_j (X_{lj} - \E[X_{lj}]) \bigg) + \sum_{l=1}^n\bigg( \sum_{i=1}^m v_i\sum_{j\neq i} A_{li}A_{lj} \bar z^*_i (\E[X_{li}] - X_{li}) \bigg) \\
&= \sum_{l=1}^n \bigg( \sum_{i=1}^m v_j \sum_{j\neq i}  A_{li}A_{lj} \bar z^*_i (X_{li} - \E[X_{li}]) \bigg) + \sum_{l=1}^n\bigg( \sum_{i=1}^m v_i\sum_{j\neq i} A_{li}A_{lj} \bar z^*_i (\E[X_{li}] - X_{li}) \bigg) \\
&= \sum_{l=1}^n \bigg( \sum_{i=1}^m (X_{li}- \E X_{li}) \sum_{j\neq i} A_{li}A_{lj} \bar z_i^* (v_j - v_i) \bigg)
\end{aligned}
\end{equation*}
\end{remark}

\section{Proofs for the decomposition approach}

Fixing an assignment $A$, we have:
\begin{equation*}
\begin{aligned}
&d\cdot\sum_{i=1}^m v_i \bigg(\sum_{j\neq i} \pi_j^*(P_{ji}-P_{ji}^*) + \pi_i^*(P_{ij}^* - P_{ij})  \bigg)\\
&= \sum_{i=1}^m v_i \bigg(\sum_{j\neq i} \bar z^*_j \big(\sum_{l=1}^n A_{li}A_{lj}X_{lj}(1-X_{li}) - \E[ A_{li}A_{lj}X_{lj}(1-X_{li})]\big) + \\
& \quad\quad\quad\sum_{j\neq i} \bar z^*_i \big(\sum_{l=1}^n  \E[ A_{li}A_{lj}X_{li}(1-X_{lj})] - A_{li}A_{lj}X_{li}(1-X_{lj})\big)  \bigg)\\
&= \sum_{i=1}^m v_i \bigg(\sum_{l=1}^n\sum_{j\neq i} \big( \bar z^*_jA_{li}A_{lj}X_{lj}(1-X_{li}) - \E[ \bar z^*_j A_{li}A_{lj}X_{lj}(1-X_{li})]\big) + \\
& \quad\quad\quad\sum_{l=1}^n\sum_{j\neq i} \big(  \E[ \bar z^*_i A_{li}A_{lj}X_{li}(1-X_{lj})] -  \bar z^*_iA_{li}A_{lj}X_{li}(1-X_{lj})\big)  \bigg)\\
&= \sum_{i=1}^m v_i \bigg(\sum_{l=1}^n\sum_{j\neq i} \big( \bar z^*_jA_{li}A_{lj}X_{lj} - \bar z^*_jA_{li}A_{lj}X_{lj}X_{li} - \bar z^*_j A_{li}A_{lj}\frac{w^*_l z^*_i}{(w_l^*+ z^*_i)(w_l^*+ z^*_j)} \big) + \\
& \quad\quad\quad\sum_{l=1}^n\sum_{j\neq i} \big(  \bar z^*_i A_{li}A_{lj}\frac{w^*_l z^*_j}{(w_l^*+ z^*_i)(w_l^*+ z^*_j)} -  \bar z^*_iA_{li}A_{li}X_{lj} +  \bar z^*_iA_{li}A_{lj}X_{lj}X_{li})\big)  \bigg)\\
&= \sum_{i=1}^m v_i \bigg(\sum_{l=1}^n\sum_{j\neq i} \big( \bar z^*_jA_{li}A_{lj}X_{lj} - \bar z^*_jA_{li}A_{lj}X_{lj}X_{li} - A_{li}A_{lj}\frac{w^*_l \bar z^*_j( z^*_i+ w_l^* - w_l^*)}{(w_l^*+ z^*_i)(w_l^*+ z^*_j)} \big) + \\
& \quad\quad\quad\sum_{l=1}^n\sum_{j\neq i} \big(  A_{li}A_{lj}\frac{w^*_l\bar z^*_i ( z^*_j+w_l^*-w_l^*) }{(w_l^*+ z^*_i)(w_l^*+ z^*_j)} -  \bar z^*_iA_{li}A_{li}X_{lj} +  \bar z^*_iA_{li}A_{lj}X_{lj}X_{li})\big)  \bigg)\\
&\text{After some rearrangment}\\
&= \sum_{i=1}^m v_i\bigg( \sum_{l=1}^n\sum_{j\neq i} A_{li}A_{lj} \bar z^*_j X_{lj} - A_{li}A_{lj} \bar z^*_j \frac{w^*_l}{w_l^* +  z^*_j}) \bigg) \\
&+ \sum_{i=1}^m v_i\bigg( \sum_{l=1}^n\sum_{j\neq i} A_{li}A_{lj} \bar z^*_i \frac{w_l^*}{w_l^* +  z^*_i} - A_{li}A_{lj} \bar z^*_iX_{li}) \bigg) \\
&+ \sum_{i=1}^m v_i\bigg( \sum_{l=1}^n\sum_{j\neq i} A_{li}A_{lj} (\bar z^*_i-\bar z^*_j) X_{li}X_{lj} - A_{li}A_{lj} (\bar z^*_i-\bar z^*_j) \frac{{w_l^*}^2}{(w_l^*+ z^*_i)(w_l^*+ z^*_j)} \bigg) \\
&= \sum_{i=1}^m v_i\bigg( \sum_{l=1}^n\sum_{j\neq i} A_{li}A_{lj} \bar z^*_j (X_{lj} - \E[X_{lj}]) \bigg)
+ \sum_{i=1}^m v_i\bigg( \sum_{l=1}^n\sum_{j\neq i} A_{li}A_{lj} \bar z^*_i (\E[X_{li}] - X_{li}) \bigg)\\
&+ \sum_{i=1}^m v_i\bigg( \sum_{l=1}^n\sum_{j\neq i} A_{li}A_{lj} (\bar z^*_i-\bar z^*_j) (X_{li}X_{lj} - \E[X_{li}X_{lj}]) \bigg) \\
&=\sum_{l=1}^n \bigg( \sum_{i=1}^m v_i \sum_{j\neq i} A_{li}A_{lj} \bar z^*_j (X_{lj} - \E[X_{lj}]) \bigg) + \sum_{l=1}^n\bigg( \sum_{i=1}^m v_i\sum_{j\neq i} A_{li}A_{lj} \bar z^*_i (\E[X_{li}] - X_{li}) \bigg) \\
&+  \sum_{l=1}^n\bigg(\sum_{i=1}^m v_i\sum_{j\neq i} A_{li}A_{lj} (\bar z^*_i-\bar z^*_j) (X_{li}X_{lj} - \E[X_{li}X_{lj}]) \bigg) \\
\end{aligned}
\end{equation*}


~\\
\textbf{Bounding the first term:} Let us bound the first term

\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n \bigg( \sum_{i=1}^m v_i \sum_{j\neq i} A_{li}A_{lj} \bar z^*_j (X_{lj} - \E[X_{lj}]) \bigg)  \\
&=\sum_{l=1}^n \sum_{j=1}^m  (X_{lj} - \E[X_{lj}]) \cdot \bigg(\sum_{i\neq j} v_i A_{li}A_{lj} \bar z^*_j  \bigg)\\
&= \sum_{l=1}^n \sum_{j=1}^m  (X_{lj} - \E[X_{lj}]) \cdot \underbrace{\bigg(A_{lj}\bar z^*_j v^\top A_l  \bigg)}_{d_{lj}}\\
\end{aligned}
\end{equation*}
One can see that conditioned on event $\A$ and for a fixed $v$ and $A$, this is a sum of $mn$ independent random variables. Thus, we can use Hoeffding to show that (with high probability)

\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n \sum_{j=1}^m  (X_{lj} - \E[X_{lj}]) \cdot {\bigg(\sum_{i\neq j} v_i A_{li}A_{lj} \bar z^*_j  \bigg)}\\
% &\lesssim \sqrt{\sum_{l, j} d_{lj}^2 }\\
&\lesssim \sqrt{\sum_{lj} A_{lj} {{\bar{z^*}}_j}^2 \cdot (v^\top A_l)^2 }\\
&\lesssim \bar z_{\max}^* \sqrt{\sum_{l} (v^\top A_l)^2 \cdot \sum_j A_{lj} }\\
&\lesssim \bar z_{\max}^* \sqrt{mp} \sqrt{\sum_{l} v^\top A_lA_l^\top v}\\
&\asymp \bar z_{\max}^* \sqrt{mp} \sqrt{\lambda_{\max}(A^\top A)} \lesssim \frac{\kappa}{m} \sqrt{mp} \sqrt{nmp^2}
\end{aligned}
\end{equation*}

The last inequality comes from
$ \lambda_{\max}(A^\top A) = \max_{v} \sum_{ij} v_i v_j B_{ij} \lesssim \max_v \{np^2 v^\top (\mb 1\mb 1^\top)v \} \lesssim mnp^2 $ and $\kappa = z^*_{\max} - z^*_{\min}$

~\\
\textbf{Bounding the second linear term:}

\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n\bigg( \sum_{i=1}^m v_i\sum_{j\neq i} A_{li}A_{lj} \bar z^*_i (\E[X_{li}] - X_{li}) \bigg) \\
&= \sum_{l=1}^n\sum_{i=1}^m (\E[X_{li}] - X_{li}) \cdot A_{li} \cdot  \bigg( v_i \bar z^*_i \sum_{j\neq i} A_{lj} \bigg) 
\end{aligned}
\end{equation*}
Again we have a sum over $mn$ independent random variables. To bound the total, we invoke Hoeffding's inequality:

\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n\sum_{i=1}^m (\E[X_{li}] - X_{li}) \cdot A_{li} \cdot  \bigg( v_i \bar z^*_i \sum_{j\neq i} A_{lj} \bigg)  \\
&\lesssim \sqrt{ \sum_{l=1}^n\sum_{i=1}^m  A_{li} \bigg( v_i \bar z^*_i \sum_{j\neq i} A_{lj} \bigg)^2 }\\
&\lesssim  \sqrt{ \sum_{l=1}^n\sum_{i=1}^m v_i^2 \bar z_{\max}^* \cdot A_{li} \bigg(\sum_{j\neq i} A_{lj} \bigg)^2 }\\
&\asymp \bar z_{\max}^* \sqrt{ \sum_{i=1}^m v_i^2  \sum_{l=1}^n A_{li}\bigg(\underbrace{\sum_{j\neq i} A_{lj}}_{\lesssim mp} \bigg)^2 }\\
&\lesssim  \bar z_{\max}^* \sqrt{ \sum_{i=1}^m v_i^2  \bigg(\underbrace{\sum_{l=1}^n A_{li}}_{\lesssim np}\cdot m^2p^2 \bigg) }\\
&\lesssim \bar z_{\max}^* \sqrt{ \sum_{i=1}^m v_i^2  \cdot np \cdot m^2p^2 } \lesssim \frac{\kappa}{m} \sqrt{mp} \cdot \sqrt{mnp^2}
% &\asymp \bar z_{\max}^* \sqrt{ \sum_{i=1}^m v_i^2 \sum_{l=1}^n \bigg(\sum_{j\neq i} A_{li} A_{lj} + 2\sum_{k\neq j\neq i} A_{lj}A_{lk}A_{li} \bigg) }\\
% &\asymp \bar z_{\max}^* \sqrt{ \sum_{i=1}^m v_i^2 \bigg(\sum_{j\neq i} \underbrace{B_{ij}}_{\asymp np^2} + 2\sum_{k\neq j\neq i} \underbrace{B_{ijk}}_{\asymp np^3} \bigg) }\\
% &\lesssim \bar z_{\max}^* \sqrt{ \sum_{i=1}^m v_i^2 \big( mnp^2 + m^2np^3\big) }\\
% &\lesssim \frac{\kappa}{m} \max\{\sqrt{mnp^2}, \sqrt{mp}\sqrt{mnp^2}\} \asymp \frac{\kappa}{m} \sqrt{mp}\sqrt{mnp^2}\\
\end{aligned}
\end{equation*}
% Assuming that $mp = \omega(1)$ then the second linear term is bounded in the same way as the first linear term, i.e., $\frac{\kappa}{m} \sqrt{mp} \sqrt{nmp^2}$

~\\
\textbf{Bounding the third quadratic term: }To use the standard Hanson-Wright's inequality (cf. \cite{rudelson2013hanson}) which applies to second order chaos of centered random variables, we first observe that:

\begin{equation*}
\begin{aligned}
&\sum_{l=1}^n\bigg(\sum_{i=1}^m v_i\sum_{j\neq i} A_{li}A_{lj} (\bar z^*_i-\bar z^*_j) (X_{li}X_{lj} - \E[X_{li}X_{lj}]) \bigg)\\
&= \sum_{l=1}^n X_l^\top M^l X_l - \E [X_l]^\top M^l \E[X_l]\\
&= \sum_{l=1}^n\bigg( {(X_l-\E[X_l])^\top M^l (X_l-\E[X_l])} + {(X_l - \E [X_l])^\top M^l \E[X_l]} + {\E[X_l]^\top M^l (X_l - \E[X_l])}\bigg) \\
&= \underbrace{ \sum_{l=1}^n(X_l-\E[X_l])^\top M^l (X_l-\E[X_l])}_{S_1} + \underbrace{ \sum_{l=1}^n(X_l - \E [X_l])^\top M^l \E[X_l]}_{S_2} + \underbrace{ \sum_{l=1}^n\E[X_l]^\top M^l (X_l - \E[X_l])}_{S_3} \\
\end{aligned}
\end{equation*}
where $X_l = (X_{li})_{i=1}^m$ and $M^l_{ij} = v_i A_{li}A_{lj} (\bar z_i^* - \bar z_j^*)$. We now bound these three terms separately.

The first term can be bounded using the standard Hanson-Wright's inequality, we first rewrite it as:
\begin{equation*}
\begin{aligned}
S_1 = \begin{bmatrix}X_1\\ \vdots \\ X_n \end{bmatrix}^\top \bigg[\diag(M^1,\ldots, M^l)  \bigg] \begin{bmatrix}X_1\\ \vdots \\ X_n\end{bmatrix}
\end{aligned}
\end{equation*}
where $M = \bigg[\diag(M^1,\ldots, M^n)  \bigg]$ is a block diagonal matrix with the $(l, l)$ blocks being $M^l$ and all other blocks being 0.
Hanson-Wright's inequality gives
$$ \Pr(\lvert S_1 \rvert > t) \lesssim \exp{-\min\{\frac{t^2}{\lVert M\rVert_F^2}, \frac{t}{\lVert M\rVert_{op}}  \}} $$
The frobenius norm term can be bounded as
\begin{equation*}
\begin{aligned}
\lVert M\rVert_F^2 &= \sum_{l=1}^n \lVert M^l \rVert_F^2= \sum_{l=1}^n \sum_{i\neq j} v_i^2 A_{li}A_{lj}(\bar z_i^* - \bar z^*_j)^2
\leq \frac{\kappa^2}{m^2} \sum_{l=1}^n\sum_{i\neq j} v_i^2 A_{li}A_{lj}\\
&=\frac{\kappa^2}{m^2}\sum_{i=1}^m v_i^2 \sum_{l=1}^n \sum_{j\neq i} A_{li}A_{lj}
= \frac{\kappa^2}{m^2} \sum_{i=1}^m v_i^2\sum_{j\neq i} B_{ij}\\
&\asymp\frac{\kappa^2}{m^2}  np^2m \sum_{i=1}^m v_i^2 \asymp\frac{\kappa^2}{m^2} mnp^2
\end{aligned}
\end{equation*}
Due to the uniform random sampling, it should be the case that $\lVert M\rVert_F \asymp \sqrt n \lVert M^l \rVert_F \gtrsim \sqrt n \lVert M^l \rVert_{op} \forall l$. Therefore, the bound is controlled by the exponential quadratic term and we have:
$$ S_1 \lesssim \sqrt{\frac{\kappa^2}{m^2}} \cdot \sqrt{mnp^2} \asymp \sqrt{\frac{np^2}{m}} $$ 

~\\
For the second and third term
\begin{equation*}
\begin{aligned}
S_2 &= \sum_{l=1}^n \bigg( \sum_{i\neq j} v_i A_{li} A_{lj} (\bar z_i^* - \bar z_j^*) (X_{li} - \E[X_{li}]) \E[X_{lj}]  \bigg)\\
&= \sum_{l=1}^n \sum_{i=1}^m (X_{li} - \E[X_{li}]) \cdot \bigg(v_i A_{li}\sum_{j\neq i} A_{lj}\E[X_{lj}]   \bigg)\\
&\text{Applying Hoeffding's inequality}\\
&\lesssim \sqrt{\sum_{l=1}^n \sum_{i=1}^m \bigg( v_i A_{li}\sum_{j\neq i} (\bar z_i^* - \bar z_j^*)A_{lj}\E[X_{lj}]   \bigg)^2 }\\
&\lesssim \sqrt{\sum_{l=1}^n \sum_{i=1}^m \bigg( v_i A_{li}\sum_{j\neq i}(\underbrace{\bar z_i^* - \bar z_j^*}_{\lesssim \frac{\kappa}{m} }) A_{lj}   \bigg)^2 }\\
&\lesssim \frac{\kappa}{m}  \sqrt{\sum_{l=1}^n \sum_{i=1}^m v^2_i A_{li} \bigg( \sum_{j\neq i} A_{lj}   \bigg)^2 }\\
&\text{Following the same argument as that for bounding the second linear term}\\
&\lesssim \frac{\kappa}{m} \sqrt{mp}\sqrt{mnp^2} 
\end{aligned}
\end{equation*}
\\

For the third term:
\begin{equation*}
\begin{aligned}
S_3 &= \sum_{l=1}^n \bigg( \sum_{i\neq j} v_i A_{li} A_{lj} (\bar z_i^* - \bar z_j^*) \E[X_{li}]  (X_{lj} - \E[X_{lj}]) \bigg)\\
&= \sum_{l=1}^n \sum_{j=1}^m (X_{lj} - \E[X_{lj}]) \bigg( \sum_{i\neq j} v_i A_{li} A_{lj} (\bar z_i^* - \bar z_j^*) \E[X_{li}]  \bigg)\\
&\text{Applying Hoeffding's inequality}\\
&\lesssim \sqrt{\sum_{l=1}^n\sum_{j=1}^m \bigg( \sum_{i\neq j} v_i A_{li} A_{lj} (\bar z_i^* - \bar z_j^*) \E[X_{li}]  \bigg)^2  }\\
&\lesssim \frac{\kappa}{m} \sqrt{\sum_{l=1}^n\sum_{j=1}^m A_{lj} \bigg( \sum_{i\neq j} v_i A_{li} \bigg)^2 }\\
&\lesssim \frac{\kappa}{m}\sqrt{\sum_{l=1}^n\sum_{j=1}^m A_{lj} \bigg( \sum_{i\neq j} v_i A_{li} \bigg)^2 }\\
&\text{Following the same argument as that for bounding the first linear term}\\
&\lesssim\frac{\kappa}{m} \sqrt{mp}\sqrt{mnp^2}
\end{aligned}
\end{equation*}


==> analysis/entrywise_analysis.tex <==
The decomposition of $\lvert \pi_i - \pi_i^*\rvert$ remains the same.
\begin{equation*}
\begin{aligned}
\pi_i - \pi_i^* &= \underbrace{\sum_{j\neq i} (\pi_j - \pi_j^*)P_{ji}}_{I_1} + \underbrace{(\pi_i - \pi_i^*)P_{ii}}_{I_2} + \underbrace{\sum_{j\neq i} \pi_j^*(P_{ji} - P^*_{ji})}_{I_3} + \underbrace{\pi_i^*(P_{ii}-P_{ii}^*)}_{I_4}\,.
\end{aligned}
\end{equation*}

\subsection{Constant or Slowly Growing $m$ Regime}
We first collect some facts from the $\ell_2$ analysis of the spectral algorithm.
\begin{theorem}\label{thm:stationary-error-bound} Suppose that $np^2 \geq \max\{C_2 \frac{12^2 e^{4\kappa}}{\gamma^2} \log m, C_1\log m\} $ for sufficiently large constants (e.g., $C_2 \geq 30$, $C_1 \geq 101$). Then
$$ \lVert \pi - \pi^* \rVert_{2} \leq \frac{48/\sqrt 3 e^{3\kappa}}{\gamma}\cdot \frac{\sqrt{ \max\{m, \log np^2  \}  } }{m\sqrt{np^2}}\, $$
and
$$ \lvert P_{ij} - P^*_{ij}\rvert  \leq \frac{\gamma np^2 }{e^{2\kappa} 8d} = \frac{\gamma}{12 m e^{2\kappa} } \quad\forall i\neq j$$
with probability at least $1- \min\{\exp{-12m}, \frac{1}{(np^2)^{12}} \} -  \exp{-\frac{\gamma^2np^2}{10 \cdot 12^2 \cdot e^{4\kappa}}} - \exp{-\frac{np^2}{20}} $. 
\end{theorem}
We also have
$$ \frac{1}{m} \leq \pi^*_{\max} = \lVert \pi^* \rVert_{\infty} \leq \frac{e^\kappa\sum_{i=1}^m \pi^*_i}{m} =\frac{e^{\kappa}}{m}\,. $$


~\\
\textbf{Bounding $I_1$}
\begin{lemma} Consider the setting of Theorem \ref{thm:stationary-error-bound}, there exists a constant $\alpha_1$ such that
$$ I_1 \leq  \alpha_1 \cdot \frac{\sqrt{ \max\{m, \log np^2  \}  } }{\sqrt{mnp^2}} \cdot \lVert \pi^*\rVert_{\infty} $$
with probability at least $1- \min\{\exp{-12m}, \frac{1}{(np^2)^{12}} \} -  \exp{-\frac{\gamma^2np^2}{10 \cdot 12^2 \cdot e^{4\kappa}}} - \exp{-\frac{np^2}{20}} $.
\end{lemma}

\begin{proof}
% \begin{equation*}
\begin{align*}
I_1 &= \sum_{j\neq i} (\pi_j - \pi^*_j) P_{ji} \\
&\text{[Using Cauchy-Schwarz]}\\
&\leq \lVert \pi - \pi^* \rVert_2 \cdot \sqrt{\sum_{j\neq i} P_{ji}^2} = \lVert \pi - \pi^* \rVert_2 \cdot \sqrt{\sum_{j\neq i} (P_{ji}- P^*_{ij} + P_{ij}^*)^2}\\
&\leq \lVert \pi - \pi^* \rVert_2 \cdot \sqrt{\sum_{j\neq i} 2(P_{ji}- P^*_{ij})^2 + 2 (P_{ij}^*)^2}\\
&\leq \lVert \pi - \pi^* \rVert_2 \cdot \sqrt 2 \cdot \sqrt{\sum_{j\neq i} \bigg( \frac{\gamma}{12 m e^{2\kappa} }\bigg)^2 + \bigg(\frac{3}{2d} {np^2}  \bigg)^2}\\
& = \lVert \pi - \pi^* \rVert_2 \cdot \sqrt 2 \cdot \sqrt{\sum_{j\neq i} \bigg( \frac{\gamma}{12 m e^{2\kappa} }\bigg)^2 + \bigg(\frac{3}{2d} {np^2}  \bigg)^2}\\
\displaybreak
&\leq \lVert \pi - \pi^* \rVert_2 \cdot \sqrt 2 \cdot \sqrt m \cdot  \sqrt{\bigg( \frac{\gamma}{12 m e^{2\kappa} }\bigg)^2 + \bigg(\frac{3}{2d} {np^2}  \bigg)^2}\\
&\leq \lVert \pi - \pi^* \rVert_2 \cdot \sqrt 2 \cdot \sqrt m \cdot \frac{1}{m} \cdot \sqrt{\frac{\gamma^2}{12^2 e^{4\kappa}} + 1}\\
&\leq \lVert \pi - \pi^* \rVert_2 \cdot \sqrt 2 \cdot \frac{1}{\sqrt m} \cdot \sqrt{\frac{\gamma^2}{12^2 e^{4\kappa}} + 1}\\
&\leq \frac{48/\sqrt 3 e^{3\kappa}}{\gamma}\cdot \frac{\sqrt{ \max\{m, \log np^2  \}  } }{m\sqrt{np^2}} \cdot \sqrt 2 \cdot \frac{1}{\sqrt m} \cdot \sqrt{\frac{\gamma^2}{12^2 e^{4\kappa}} + 1}\\
&\leq \underbrace{\frac{48/\sqrt 3 e^{3\kappa}}{\gamma}\cdot \sqrt 2 \cdot \sqrt{\frac{\gamma^2}{12^2 e^{4\kappa}} + 1}}_{\alpha_1} \cdot \frac{\sqrt{ \max\{m, \log np^2  \}  } }{\sqrt{mnp^2}} \cdot \lVert \pi^*\rVert_{\infty}\\
&= \alpha_1 \cdot \frac{\sqrt{ \max\{m, \log np^2  \}  } }{\sqrt{mnp^2}} \cdot \lVert \pi^*\rVert_{\infty}\,.
\end{align*}
\end{proof}

~\\
\textbf{Bounding $I_2$}
\begin{lemma} Consider the setting of Theorem \ref{thm:stationary-error-bound}. There exists a constant $\alpha_2 < 1$ such that
$$ I_2 \leq \alpha_2 \cdot \lVert \pi - \pi \rVert_{\infty}  $$
with probability at least $1- \min\{\exp{-12m}, \frac{1}{(np^2)^{12}} \} -  \exp{-\frac{\gamma^2np^2}{10 \cdot 12^2 \cdot e^{4\kappa}}} - \exp{-\frac{np^2}{20}} $.
\end{lemma}

\begin{proof} It suffices to bound $P_{ii}$ away from 1.
\begin{align*}
\lvert P_{ii} - P^*_{ii}\rvert &= \bigg\lvert\sum_{j\neq i} P^*_{ij} - P_{ij}\bigg\rvert \\
&\leq \sum_{j\neq i} \lvert P_{ij}^* - P_{ij}\rvert \\
&\leq \frac{\gamma}{12 e^{2\kappa}}\,.
\end{align*}
On the other hand, $P_{ii}^* = 1- \frac{1}{d} \cdot\sum_{j\neq i} P_{ij}^* \leq 1- \frac{3}{2d}\gamma mnp^2 = 1- \gamma$. We have
$$ P_{ii} \leq 1- \gamma + \frac{\gamma}{12e^{2\kappa}} < 1 =: \alpha_2 $$
\end{proof}

~\\
\textbf{Bounding $I_3$} 
\begin{lemma} Consider the setting of Theorem \ref{thm:stationary-error-bound}. There exists a constant $\alpha_3$ such that
$$ I_3 \leq \alpha_3 \cdot   \frac{\lVert \pi^*\rVert_{\infty} \sqrt{\log np^2} }{\sqrt{np^2}} $$
with probability at least $1- \min\{\exp{-12m}, \frac{3}{(np^2)^{12}} \} -  \exp{-\frac{\gamma^2np^2}{10 \cdot 12^2 \cdot e^{4\kappa}}} - \exp{-\frac{np^2}{20}} $.
\end{lemma}

\begin{proof}
\begin{equation*}
\begin{aligned}
I_3 &= \sum_{j\neq i} \pi_j^* (P_{ji} - P_{ji}^*) = \frac{1}{d} \cdot \sum_{j\neq i}\pi_j^* \cdot \sum_{l=1}^n A_{li}A_{lj} \big[X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})] \big] \,.\\
\end{aligned}
\end{equation*}
Informally speaking, for a fixed $l$ if we change $X_{li}$, the sum above changes by at most $\frac{1}{d} \cdot \sum_{j\neq i} \pi_j^* A_{li} A_{lj} $. For a fixed $l$ and $j\neq i$, if we change $X_{lj}$, the sum above changes by at most $\frac{1}{d} \cdot \pi_j^* A_{li}A_{lj} \leq \frac{1}{d}\cdot \lVert \pi^*\rVert_{\infty} A_{li}A_{lj}$. Note also that by Cauchy-Schwarz,
\begin{equation*}\label{eqn:bounded-difference} \sum_{j\neq i} \pi_j^* A_{li} A_{lj} \leq \lVert \pi^*\rVert_{\infty} \cdot \sqrt{m-1} \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj}} \,. 
\end{equation*}
Ignore the factor $d$ for now. Hoeffding's inequality then tells us that
\begin{equation*}
\begin{aligned}
&\Pr\bigg(\sum_{j\neq i}\pi_j^* \cdot \sum_{l=1}^n A_{li}A_{lj} \big[X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})]\big] > t\,\lvert\, \A  \bigg) \\
&\leq 2\exp{-\frac{2t^2}{ \lVert \pi^*\rVert^2_{\infty} \cdot (m-1) \cdot \sum_{j\neq i}\sum_{l=1}^n A_{li}A_{lj} + \sum_{j\neq i}\sum_{l=1}^n\lVert \pi^*\rVert^2_{\infty} A_{li}A_{lj} }}\\
&\leq 2\exp{-\frac{2t^2}{ \lVert \pi^*\rVert^2_{\infty} \cdot \big(  m \sum_{j\neq i} \sum_{l=1}^n A_{li}A_{lj} \big)}}\\
&\leq 2\exp{-\frac{2t^2}{ m \lVert \pi^*\rVert^2_{\infty} \cdot 3/2mnp^2 }}\\
\end{aligned}
\end{equation*}
Set $t = \sqrt{12} \cdot \sqrt{\frac{3}{8}} \cdot m \sqrt{np^2} \cdot \sqrt{\log np^2} \cdot \lVert \pi^*\rVert_{\infty} $. We have 
$$ I_3 \leq \frac{1}{d} \cdot \sqrt{12} \cdot \sqrt{\frac{3}{8}} \cdot m \sqrt{np^2} \cdot \sqrt{\log np^2} \cdot \lVert \pi^*\rVert_{\infty}  = \sqrt 2 \cdot \frac{\lVert \pi^*\rVert_{\infty} \sqrt{\log np^2} }{\sqrt{np^2}} $$ 
with probability at least $1 - \frac{2}{(np^2)^{12}}$.
\end{proof}

~\\
\textbf{Bounding $I_4$}
\begin{lemma} Consider the setting of Theorem \ref{thm:stationary-error-bound}. There exists a constant $\alpha_4$ such that
$$ I_4 \leq \alpha_4 \cdot   \frac{\lVert \pi^*\rVert_{\infty} \sqrt{\log np^2} }{\sqrt{np^2}} $$
with probability at least $1- \min\{\exp{-12m}, \frac{3}{(np^2)^{12}} \} -  \exp{-\frac{\gamma^2np^2}{10 \cdot 12^2 \cdot e^{4\kappa}}} - \exp{-\frac{np^2}{20}} $.
\end{lemma}

\begin{proof}
\begin{equation*}
\begin{aligned}
I_4 &= \sum_{j\neq i} \pi_i^* (P_{ij}^* - P_{ij} ) = \frac{1}{d} \cdot \sum_{j\neq i}\pi_i^* \cdot \sum_{l=1}^n A_{li}A_{lj} \big[\E[X_{li}(1-X_{lj}) - X_{li}(1-X_{lj}) \big] \,,\\
\end{aligned}
\end{equation*}
which has essentially the same form as $I_3$. Following the same argument as that in the proof of the third claim, we can bound $I_4$ as
$$ I_4 \leq \frac{1}{d} \cdot \sqrt{12} \cdot \sqrt{\frac{3}{8}} \cdot m \sqrt{np^2} \cdot \sqrt{\log np^2} \cdot \lVert \pi^*\rVert_{\infty}  = \sqrt 2 \cdot \frac{\lVert \pi^*\rVert_{\infty} \sqrt{\log np^2} }{\sqrt{np^2}} $$ 
with probability at least $1 - \frac{2}{(np^2)^{12}}$.
\end{proof}


~\\
\textbf{Putting the terms together}, we have 
$$ \lvert \pi_i - \pi_i^*\rvert_{\infty} \leq \alpha_2 \cdot \lVert \pi - \pi^*\rVert_{\infty} + (\alpha_1 + \alpha_3 + \alpha_4) \cdot \frac{\sqrt{ \log np^2   } }{\sqrt{np^2}} \cdot \lVert \pi^*\rVert_{\infty}\,. $$
Rearranging the term and maximizing the LHS gives
$$ \frac{ \lVert \pi - \pi^*\rVert_{\infty} }{ \lVert \pi^*\rVert_{\infty}  } \leq \frac{\alpha_1 + \alpha_3 + \alpha_4}{1-\alpha_2} \cdot \frac{\sqrt{ \log np^2  } }{\sqrt{np^2}} \,. $$

\newpage
\subsection{Large $m$ Regime}
Recall the following results from our $\ell_2$ analysis under large $m$ regime.
\begin{theorem}\label{thm:stationary-error-bound-growing-m} Suppose that $np^2 \geq \max\{C_2 \frac{12^2 e^{4\kappa}}{\gamma^2} \log m, C_1\log m\} $ and that $mp \geq C''\log m$ for sufficiently large constants $C_1, C_2, C''$ (e.g., $C_2 \geq 30$, $C_1, C'' \geq 101 $). Then the output of the spectral algorithm satisfies
$$ \lVert \pi - \pi^* \rVert_2 \leq \frac{48/\sqrt{2} e^{3\kappa}}{\gamma} \cdot \frac{1}{\sqrt{mnp}} $$
with probability at least $1- \exp{-12m} - \exp{-\frac{\gamma^2np^2}{10 \cdot 12^2 \cdot e^{4\kappa}}} - n^{-9}$.
\end{theorem}

Note that the bound on $I_2$ doesn't change. We, however, obtain sharper bounds for $I_1, I_3, I_4$.

~\\
\textbf{Sharper Bound on $I_1$}
\begin{lemma} Consider the setting of Theorem \ref{thm:stationary-error-bound-growing-m}, there exists a constant $\alpha'_1$ such that
$$ I_1 \leq  \alpha'_1 \cdot \frac{1}{\sqrt{mnp}} \cdot \lVert \pi^*\rVert_{\infty} $$
with probability at least $1- \exp{-12m} - \exp{-\frac{\gamma^2np^2}{10 \cdot 12^2 \cdot e^{4\kappa}}} - n^{-9}$.
\end{lemma}

\begin{proof} Following the same decomposition as in the proof of the bound on $I_1$ under the constant (or small) $m$ regime,
\begin{align*}
I_1 &\leq \lVert \pi - \pi^* \rVert_2 \cdot \sqrt 2 \cdot \frac{1}{\sqrt m} \cdot \sqrt{\frac{\gamma^2}{12^2 e^{4\kappa}} + 1}\\
&\leq \frac{48/\sqrt 2 e^{3\kappa}}{\gamma}\cdot \frac{1 }{m\sqrt{np}} \cdot \sqrt 2 \cdot \frac{1}{\sqrt m} \cdot \sqrt{\frac{\gamma^2}{12^2 e^{4\kappa}} + 1}\\
&\leq \underbrace{\frac{48/\sqrt 2 e^{3\kappa}}{\gamma}\cdot \sqrt 2 \cdot \sqrt{\frac{\gamma^2}{12^2 e^{4\kappa}} + 1} }_{\alpha'_1} \cdot \frac{1}{\sqrt{mnp} \cdot \lVert \pi^*\rVert_{\infty}}\\
&= \frac{\alpha'_1}{\sqrt{mnp}} \cdot \lVert \pi^*\rVert_{\infty}\,.
\end{align*}
\end{proof}

~\\
\textbf{Sharper Bound on $I_3$} 
\begin{lemma} Consider the setting of Theorem \ref{thm:stationary-error-bound-growing-m}. There exists a constant $\alpha'_3$ such that
$$ I_3 \leq \alpha'_3 \cdot   \frac{\lVert \pi^*\rVert_{\infty} \sqrt{\log np} }{\sqrt{np}} $$
with probability at least $1- \exp{-12m} - \exp{-\frac{\gamma^2np^2}{10 \cdot 12^2 \cdot e^{4\kappa}}} - n^{-9}$.
\end{lemma}

\begin{proof}
\begin{equation*}
\begin{aligned}
I_3 &= \sum_{j\neq i} \pi_j^* (P_{ji} - P_{ji}^*) = \frac{1}{d} \cdot \sum_{j\neq i}\pi_j^* \cdot \sum_{l=1}^n A_{li}A_{lj} \big[X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})] \big] \,.\\
\end{aligned}
\end{equation*}
Informally speaking, for a fixed $l$ if we change $X_{li}$, the sum above changes by at most $\frac{1}{d} \cdot \sum_{j\neq i} \pi_j^* A_{li} A_{lj} $. For a fixed $l$ and $j\neq i$, if we change $X_{lj}$, the sum above changes by at most $\frac{1}{d} \cdot \pi_j^* A_{li}A_{lj} \leq \frac{1}{d}\cdot \lVert \pi^*\rVert_{\infty} A_{li}A_{lj}$. Note also that by Cauchy-Schwarz and under the growing $m$ regime,
\begin{equation*}
\begin{aligned}
&\sum_{j\neq i} \pi_j^* A_{li} A_{lj} \leq \lVert \pi^*\rVert_{\infty} \cdot \sum_{j\neq i} A_{lj} \cdot A_{li}A_{lj}  \\
&\leq \lVert \pi^*\rVert_{\infty} \cdot \sqrt{\sum_{j\neq i} A_{lj} } \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj} }\\
&\leq \lVert \pi^*\rVert_{\infty} \cdot \sqrt{3/2} \cdot \sqrt{mp} \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj} } \,.\\
\end{aligned}
\end{equation*}
We have
\begin{equation*}
\begin{aligned}
&\Pr\bigg(\sum_{j\neq i}\pi_j^* \cdot \sum_{l=1}^n A_{li}A_{lj} \big[X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})]\big] > t\,\lvert\, \A^+  \bigg) \\
&\leq 2\exp{-\frac{2t^2}{ m \lVert \pi^*\rVert^2_{\infty} \cdot 9/4\cdot mp \cdot np^2 }}\\
\end{aligned}
\end{equation*}
Set $t = \sqrt{12} \cdot \sqrt{\frac{9}{8}} \cdot m \sqrt{np} \cdot \sqrt{\log np^2} \cdot \lVert \pi^*\rVert_{\infty} $. We have 
$$ I_3 \leq \frac{1}{d} \cdot \sqrt{12} \cdot \sqrt{\frac{9}{8}} \cdot m \sqrt p \cdot \sqrt{np^2} \cdot \sqrt{\log np^2} \cdot \lVert \pi^*\rVert_{\infty}  = \sqrt{27/2} \cdot \frac{\lVert \pi^*\rVert_{\infty} \sqrt{\log np} }{\sqrt{np}} $$ 
with probability at least $1 - \frac{2}{(np)^{12}}$.
\end{proof}

~\\
\textbf{Sharper Bound on $I_4$}
\begin{lemma} Consider the setting of Theorem \ref{thm:stationary-error-bound-growing-m}. There exists a constant $\alpha'_4$ such that
$$ I_4 \leq \alpha'_4 \cdot   \frac{\lVert \pi^*\rVert_{\infty} \sqrt{\log np} }{\sqrt{np}} $$
with probability at least $1- \exp{-12m} - \exp{-\frac{\gamma^2np^2}{10 \cdot 12^2 \cdot e^{4\kappa}}} - n^{-9}$.
\end{lemma}

\begin{proof}
The proof is omitted.
\end{proof}


~\\
\textbf{Putting the terms together}, we have under the growing $m$ regime,
$$ \frac{ \lVert \pi - \pi^*\rVert_{\infty} }{ \lVert \pi^*\rVert_{\infty}  } \leq \frac{\alpha_1 + \alpha_3 + \alpha_4}{1-\alpha_2} \cdot \frac{\sqrt{ \log np  } }{\sqrt{np}} \,. $$


==> analysis/entrywise_analysis_informal.tex <==
Pick an index $i \in [m]$.
\begin{equation*}
\begin{aligned}
\pi_i - \pi_i^* &= (\pi^\top P)_i - ({\pi^*}^\top P^* )_i\\
&= \sum_j \pi_j P_{ji} - \sum_j \pi_j^* P_{ji}^*\\
&= \sum_j \pi_j P_{ji} - \sum_j \pi_j^*(P_{ji}^* - P_{ji} + P_{ji})\\
&= \sum_j (\pi_j - \pi_j^*)P_{ji} - \sum_j \pi_j^*(P^*_{ji} - P_{ji})\\
&= \sum_j (\pi_j - \pi_j^*)P_{ji} + \sum_j \pi_j^*(P_{ji} - P^*_{ji})\,.\\
&= \underbrace{\sum_{j\neq i} (\pi_j - \pi_j^*)P_{ji}}_{I_1} + \underbrace{(\pi_i - \pi_i^*)P_{ii}}_{I_2} + \underbrace{\sum_{j\neq i} \pi_j^*(P_{ji} - P^*_{ji})}_{I_3} + \underbrace{\pi_i^*(P_{ii}-P_{ii}^*)}_{I_4}\,.
\end{aligned}
\end{equation*}

We claim that
\begin{itemize}
\item $$ I_1 \lesssim \frac{\lVert \pi^*\rVert_{\infty}}{\sqrt{np^2}}\,, $$
\item $$ I_2 \leq c \cdot \lVert \pi - \pi^*\rVert_{\infty}\,, $$
where $c$ is some constant less than 1,
\item $$ I_3, I_4 \lesssim \frac{\lVert \pi^* \rVert_{\infty}}{\sqrt{np^2}} \,.$$
\end{itemize}

~\\
From our analysis of $\lVert \pi - \pi^* \rVert_2$, we have
$$ \lVert \pi - \pi^* \rVert_2 \lesssim \frac{\sqrt{m}\lVert \pi^*\rVert_{\infty}}{\sqrt{np^2}} \asymp \frac{1}{\sqrt{mnp^2}} \,.$$

~\\
\textbf{To prove the first claim}, first note that given $np^2 \geq C \log m$ for a sufficiently large constant $C$, then $P_{ij} = \frac{1}{d} \cdot \sum_{l=1}^n A_{li}A_{lj} X_{li}(1-X_{lj}) \lesssim \frac{np^2}{d}$. Then
\begin{equation*}
\begin{aligned}
I_1 &= \sum_{j\neq i} (\pi_j - \pi^*_j) P_{ji} \\
&\text{[Using Cauchy-Schwarz]}\\
&\leq \lVert \pi - \pi^* \rVert_2 \cdot \sqrt{\sum_{j\neq i} P_{ji}^2} \lesssim \lVert \pi - \pi^* \rVert_2 \cdot \sqrt{ \sum_{j\neq i} \bigg(\frac{np^2}{d}\bigg)^2 }\\
&\asymp \frac{\lVert \pi - \pi^* \rVert_2}{d} \cdot \sqrt m \cdot np^2 \lesssim \frac{\lVert \pi^*\rVert_{\infty}}{\sqrt{np^2} }\,.
\end{aligned}
\end{equation*}

~\\
\textbf{To prove the second claim,} it suffices to bound $P_{ii}$ away from 1 by a constant. We know that given $np^2 \geq C' \frac{\log m}{\epsilon^2}$ for some sufficiently large constant $C'$, then $\lvert P_{ij} - P_{ij}^*\rvert \leq \frac{\epsilon np^2}{d}$ and
\begin{equation*}
\begin{aligned}
\lvert P_{ii} - P^*_{ii}\rvert &= \lvert\sum_{j\neq i} P^*_{ij} - P_{ij}\rvert &\leq \sum_{j\neq i} \lvert P_{ij}^* - P_{ij}\rvert
&\lesssim \frac{\epsilon mnp^2}{d} \asymp \epsilon\,.
\end{aligned}
\end{equation*}
Given sufficiently large normalization constant $d$, $P_{ii}^* = 1- \frac{1}{d} \cdot\sum_{j\neq i} P_{ij}^* \lesssim 1- \frac{1}{d}\gamma mnp^2 \asymp 1- \gamma$. For a sufficiently small $\epsilon$, then
$$ P_{ii} \leq 1- \gamma + \epsilon \,.$$

~\\
\textbf{To prove the third claim}, we will use Hoeffding's inequality. Firsly, note that
\begin{equation*}
\begin{aligned}
I_3 &= \sum_{j\neq i} \pi_j^* (P_{ji} - P_{ji}^*) = \frac{1}{d} \cdot \sum_{j\neq i}\pi_j^* \cdot \sum_{l=1}^n A_{li}A_{lj} \big[X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})] \big] \,.\\
\end{aligned}
\end{equation*}
Informally speaking, for a fixed $l$ if we change $X_{li}$, the sum above changes by at most $\frac{1}{d} \cdot \sum_{j\neq i} \pi_j^* A_{li} A_{lj} $. Note that by Cauchy-Schwarz,
\begin{equation}\label{eqn:bounded-difference} \sum_{j\neq i} \pi_j^* A_{li} A_{lj} \leq \lVert \pi^*\rVert_{\infty} \cdot \sqrt{m-1} \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj}} \,. \end{equation}
For a fixed $l$ and $j\neq i$, if we change $X_{lj}$, the sum above changes by at most $\pi_j^* A_{li}A_{lj} \leq \lVert \pi^*\rVert_{\infty} A_{li}A_{lj}$. Hoeffding's inequality then tells us that
\begin{equation*}
\begin{aligned}
I_3 &= \frac{1}{d} \sum_{j\neq i}\pi_j^* \cdot \sum_{l=1}^n A_{li}A_{lj} \big[X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})] \big] \\
&\lesssim \frac{1}{d} \cdot \sqrt{ \lVert \pi^*\rVert^2_{\infty} \cdot (m-1) \cdot \sum_{j\neq i}\sum_{l=1}^n A_{li}A_{lj} + \sum_{j\neq i}\sum_{l=1}^n\lVert \pi^*\rVert^2_{\infty} A_{li}A_{lj}  }\\
&\asymp \frac{\lVert \pi^*\rVert_{\infty} }{d} \cdot \sqrt{m \sum_{j\neq i} \sum_{l=1}^n A_{li}A_{lj} }\\
&\lesssim \frac{\lVert \pi^*\rVert_{\infty} }{d} \cdot \sqrt m \cdot \sqrt{m np^2} \asymp \frac{\lVert \pi^*\rVert_{\infty} }{\sqrt{np^2}}
\end{aligned}
\end{equation*}

~\\
\textbf{To prove the fourth claim}, similarly to the third claim, we will also use Hoeffding's inequality. Note that
\begin{equation*}
\begin{aligned}
I_4 &= \sum_{j\neq i} \pi_i^* (P_{ij}^* - P_{ij} ) = \frac{1}{d} \cdot \sum_{j\neq i}\pi_i^* \cdot \sum_{l=1}^n A_{li}A_{lj} \big[\E[X_{li}(1-X_{lj}) - X_{li}(1-X_{lj}) \big] \,,\\
\end{aligned}
\end{equation*}
which has essentially the same form as $I_3$. Following the same argument as that in the proof of the third claim, we can bound $I_4$ as
$$ I_4 \lesssim \frac{\lVert \pi^*\rVert_{\infty} }{\sqrt{np^2}}\,.$$

~\\
\textbf{Putting the claims together}, we have
$$ \lvert \pi_i - \pi^*\rvert \leq c \lVert \pi - \pi^* \rVert_{\infty} + \frac{C\lVert \pi^*\rVert_{\infty}}{ \sqrt{np^2}}\,, $$
where $c < 1$ and $C$ is some constant. Maximizing with respect to $i$ on the LHS and rearranging the terms gives us
$$ \frac{\lVert \pi - \pi^*\rVert_{\infty}}{\lVert \pi^*\rVert_{\infty}} \lesssim \frac{1}{\sqrt{np^2}}\,, $$
which seems to be the optimal rate.



\subsection{Entrywise Error Bounds for the Growing $m$ Regime}
Consider the case when $mp \gtrsim \log n$. Now follow the same decomposition as in our analysis in the previous section. 
We claim that when $m$ grows,
\begin{itemize}
\item $$ I_1 \lesssim \frac{\lVert \pi^*\rVert_{\infty}}{\sqrt{np}}\,, $$
\item $$ I_2 \leq c \cdot \lVert \pi - \pi^*\rVert_{\infty}\,, $$
where $c$ is some constant less than 1,
\item $$ I_3, I_4 \lesssim \frac{\lVert \pi^* \rVert_{\infty}}{\sqrt{np}} \,.$$
\end{itemize}
Note that similarly to the $\ell_2$ analysis of the spectral method, we also remove a $\sqrt p$ factor in the three terms $I_1, I_3, I_4$. 

~\\
\textbf{Improving term $I_1$:} We have from our $\ell_2$ analysis that when $m$ grows, 
$$ \lVert \pi - \pi^* \rVert_2 \lesssim \frac{1}{\sqrt{mnp}} \asymp \frac{\sqrt m \cdot \lVert \pi^* \rVert_{\infty} }{\sqrt{np}} \,.$$
We can then bound $I_1$ as
$$ I_1 \lesssim \frac{\lVert \pi - \pi^* \rVert_2}{d} \cdot \sqrt m \cdot np^2 \lesssim \frac{\lVert \pi^*\rVert_{\infty} }{\sqrt{np}}\,.  $$

~\\
\textbf{Improving terms $I_3$ and $I_4$:} Using the same trick that we use in our $\ell_2$ analysis of the spectral algorithm where can obtain a tighter bound on the bounded difference term in Equation (\ref{eqn:bounded-difference}) by introducing an extra $\sqrt p$ factor.
\begin{equation*}
\begin{aligned}
&\sum_{j\neq i} \pi_j^* A_{li} A_{lj} \leq \lVert \pi^*\rVert_{\infty} \cdot \sum_{j\neq i} A_{lj} \cdot A_{li}A_{lj}  \\
&\leq \lVert \pi^*\rVert_{\infty} \cdot \sqrt{\sum_{j\neq i} A_{lj} } \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj} }\\
&\leq \lVert \pi^*\rVert_{\infty} \cdot \sqrt{mp} \cdot \sqrt{\sum_{j\neq i} A_{li}A_{lj} }\\
\end{aligned}
\end{equation*}
We can thus bound $I_3$ more tightly as
\begin{equation*}
\begin{aligned}
I_3 &= \frac{1}{d} \sum_{j\neq i}\pi_j^* \cdot \sum_{l=1}^n A_{li}A_{lj} \big[X_{lj}(1-X_{li}) - \E[X_{lj}(1-X_{li})] \big] \\
&\lesssim \frac{1}{d} \cdot \sqrt{ \lVert \pi^*\rVert^2_{\infty} \cdot mp \cdot \sum_{j\neq i}\sum_{l=1}^n A_{li}A_{lj} + \sum_{j\neq i}\sum_{l=1}^n\lVert \pi^*\rVert^2_{\infty} A_{li}A_{lj}  }\\
&\asymp \frac{\lVert \pi^*\rVert_{\infty} }{d} \cdot \sqrt{mp \sum_{j\neq i} \sum_{l=1}^n A_{li}A_{lj} }\\
&\lesssim \frac{\lVert \pi^*\rVert_{\infty} }{d} \cdot \sqrt{mp} \cdot \sqrt{m np^2} \asymp \frac{\lVert \pi^*\rVert_{\infty} }{\sqrt{np}}
\end{aligned}
\end{equation*}
Since the terms $I_3$ and $I_4$ can be bounded in the same way, we also obtain tighter rate for $I_4$.

~\\
\textbf{Putting all the terms together,} we have
$$ \frac{\lVert \pi - \pi^*\rVert_{\infty}}{\lVert \pi^*\rVert_{\infty}} \lesssim \frac{1}{\sqrt{np}}\, $$
under the regime where $mp \gtrsim \log n$.


==> analysis/lower_bound_all_estimators.tex <==
\textbf{Large $m$ regime.}

\begin{theorem}\label{thm:lower-bound-all-estimators} There exists a class of Rasch models such that for any statistical estimator $\hat\beta$, the minimax risk is lower bounded as
$$ \E \lVert\hat \beta - \beta^* \rVert_2^2 \gtrsim \frac{m}{np}\,. $$
\end{theorem}
We will use a the packing set construction like in the proof of Theorem 1 of \cite{shah2015estimation}, coupled with the pairwise Fano's inequality for minimax lower bound.

\begin{lemma}\label{lem:fanos-minimax} (Pairwise Fano minimax lower bound) Suppose that we can construct a set $\calW = \{\beta^1, \ldots, \beta^M\}$ with cardinality $M$ such that 
$$ \max_{a\neq b\in[M]}\lVert \beta^a - \beta^b \rVert_2^2 \leq \delta^2 \quad\text{and}\quad \max_{a\neq b\in [M]}\kl(\Pr^a(X)\lVert \Pr^b(X)) \leq \beta\,. $$
Then the minimax risk is lower bounded as
$$ \inf_{\hat\beta} \sup_{\beta^* \in \calW} \E[\lVert \hat\beta - \beta\rVert_2^2] \geq \frac{\delta^2}{2}\bigg(1-\frac{\beta+\log 2}{\log M}\bigg)\,, $$
where $\hat\beta$ is the output of any estimator.
\end{lemma}

\begin{lemma}\label{lem:packing-set-shah} (Lemma 7 of \cite{shah2015estimation}) For any $\alpha \in (0, \frac{1}{4})$, there exists a set of $M(\alpha) = \theta(\exp{m})$ binary vectors $\{z^1, \ldots, z^{M(\alpha)}\} \subset \{0, 1\}^m $ such that
\begin{equation*}
\begin{aligned}
\alpha m \leq \lVert z^{a} - z^b \rVert_2^2 \leq m\quad &\forall a \neq b\in [1,\ldots, M(\alpha)] \,.\\
% z_1^a = 0 \quad &\forall a \in [1,\ldots, M(\alpha)]\,.
\end{aligned}
\end{equation*}
\end{lemma}

Consider a packing set $\{z^1, \ldots, z^{M(\alpha)}\} \subset \{0, 1\}^m $ of $m$-dimensional binary vectors given by Lemma \ref{lem:packing-set-shah}. Let
$$ \beta^a = \frac{\delta}{\sqrt m} \cdot z^a \quad \forall a\in [M(\alpha)]\,, $$
where $\delta$ is to be detemined later. It is easy to see that for $a\neq b \in [M(\alpha)]$
$$  \lVert \beta^a - \beta^b \rVert_2^2 = \frac{\delta^2}{m} \cdot \lVert z^a - z^b \rVert^2_2 \leq \delta^2 \,.$$

Similar to the lower bound based on Fisher's information. Let us assume that we know exactly the parameters of the users. More over, consider the case where $\theta_1 = \ldots = \theta_n = \frac{1}{2}$.

\begin{lemma}\label{lem:kl-div-theta-known} Suppose that all of the users have parameter $\theta = \frac{1}{2}$ for all $i \in [n]$. Consider any two alternative parameter sets $\beta^a$ and $\beta^2$.
$$\kl(\Pr^a(X)\lVert \Pr^b(X)) \leq \frac{2np}{c} \cdot \lVert \beta^a - \beta^b \rVert_2^2 \leq \frac{2np\delta^2}{c} \,. $$
\end{lemma}

\begin{proof}
As a short hand notation, define $\Pr_i^a := \frac{e^{\theta}}{e^{\theta} + e^{\beta^a_i}}$ and analogously for $\Pr_i^b$. Let $c = \frac{\sqrt e}{\sqrt e + e} $.
\begin{equation*}
\begin{aligned}
\kl(\Pr^a(X)\lVert \Pr^b(X)) &= \sum_{l=1}^n \sum_{i=1}^m \kl(\Pr^a(X_{li})\lVert \Pr^b(X_{li})) \\
&= np \sum_{i=1}^m \kl(\Pr^a \lVert \Pr^b)\\
&\text{[Using the inverse Pinsker's inequality]}\\
&\leq np \sum_{i=1}^m \frac{1}{c} \cdot (\Pr_i^a - \Pr^b_i)^2\\
&\leq \frac{np}{c} \sum_{i=1}^m 2(\beta_i^a - \beta_i^b)^2\\
&= \frac{2np}{c} \cdot \lVert \beta^a - \beta^b \rVert_2^2\,.
\end{aligned}
\end{equation*}
\end{proof}

~\\
We can now apply Lemma \ref{lem:fanos-minimax}. The minimax risk is lower bounded as
$$  \inf_{\hat\beta} \sup_{\beta^* \in \calW} \E[\lVert \hat\beta - \beta\rVert_2^2] \geq \frac{\delta^2}{2}\bigg(1-\frac{Cnp\delta^2 +\log 2}{m}\bigg)\,, $$
where $C$ is some constant to be determined. Setting $\delta = \frac{\epsilon\sqrt m}{\sqrt{np}}$ for a sufficiently small $\epsilon$ gives us
$$ \inf_{\hat\beta} \sup_{\beta^* \in \calW} \E[\lVert \hat\beta - \beta\rVert_2^2] \gtrsim \frac{m}{np}\,.  $$

~\\
\textbf{Small $m$ Regime.} If we follow a similar argument as in the lower bound above for the large $m$ regime, we would need to upper bound the KL divergence between any two alternative models as $np^2\delta^2$. That is, it is a factor of $\frac{1}{p}$ smaller than the KL divergence in the large $m$ regime. A convenient fact that we get from the lower bound above is that the KL divergence between alternative models can be decomposed as a sum over all the user-item responses.
$$\kl(\Pr^a \lVert \Pr^b) = \sum_{l=1}^n \sum_{i=1}^m \, \underbrace{ \kl(\Pr^a(X_{li}) \rVert \Pr^b(X_{li} ))  }_{p\cdot  \kl(\Pr^a(X_{li}\rVert X_{li} \neq * ) \rVert \Pr^b(X_{li}\rVert X_{li} \neq * ))} \,. $$
One idea is to design the packing set such that the set of $n$ users is partitioned into two groups of users: the `informative' users and the `uninformative' users. Informative users have user parameter $\frac{1}{2}$ and uninformative users have user parameter $L$ for $L$ to be determined. For an informative user $l$ responding to an item $i$, we can follow the same argument as in the lower bound in the large $m$ regime and obtain 
$$ \kl(\Pr^a(X_{li}) \rVert \Pr^b(X_{li})) \leq p\delta^2 \,.$$
On the other hand, the notion of `uninformative-ness' can be captured by setting $L$ to be a large positive or large negative numbers. Intuitively, when a user $l$ either has a very positive or negative user parameter $\theta_l$, the response to an item $i$, $X_{li}$, is either $1$ with very high probability or $0$ with very high probability (for any value of $\beta_i$). Consequently, the KL divergence between two alternative model will be small. For a positive $\epsilon > 0$, by setting $L$ large enough, one can bound
$$ \kl(\Pr^a(X_{li}) \lVert \Pr^b (X_{li}) ) \leq p\epsilon\delta^2\,. $$
Let $S$ denote the set of informative users and $S^c$ the set of uninformative users. We have
$$ \kl(\Pr^a\lVert \Pr^b) \asymp \lvert S\rvert \cdot p\delta^2 + \lvert S^c \rvert \cdot p\epsilon\delta^2\,.  $$
One way to achieve the desired $np^2\delta^2$ rate is to set $\lvert S \rvert = np$ and choosing $\theta_l$ such that $\epsilon = p$. 

However, the limitation of this approach is that the model construction depends on the parameter $p$ itself. Note that in the error bound of the spectral method, there is a $\gamma$ factor which is $\min_{ l\in[n], i\neq j\in [m]} \Pr(X_{li}=1, X_{li}=0)$. If we choose $\epsilon = p$, then there will be a relation between $\gamma$ and $p$. This will lead to a worse upper bound.

==> analysis/preliminary_analysis.tex <==
\section{Preliminary analysis}


$d_i$ is a normalization factor to ensure that we have a valid probability transition matrices, that is $d_i$ must be sufficiently large such that:
$$\sum_{j\neq i} \frac{1}{d_i} B_{ij} = \frac{1}{d_i} \sum_{j=1, j\neq i}^m \sum_{l=1}^n A_{li}A_{lj} X_{li}(1-X_{lj}) \leq 1$$
Suppose that for each student, she is given problem $i$ with probability $p$ independently of other students and problems.


\begin{lemma} For any $i \neq j \in [m]$
$$ \Pr( \lvert P_{ij} - P^*_{ij}\rvert > t) \leq 2\exp{-\frac{t^2d^2}{ 2\bigg(\sum_{l=1}^n \big[\frac{p^2w^*_l}{(w^*_l+z^*_i)(w_l+z^*_j)}\big] +  \frac{td}{3} \bigg) }} $$
\end{lemma}

\begin{proof}
By definition we have:
\begin{equation*}
\begin{aligned}
P_{ij} - P^*_{ij} &= \frac{1}{d} \sum_{l=1}^n \underbrace{A_{li}A_{lj} X_{li}(1-X_{lj})}_{Y_{ij}^{l}\leq 1 } - \E[A_{li}A_{lj} X_{li}(1-X_{lj}) ]\\
\end{aligned}
\end{equation*}
Note that the above sum is over $n$ independent centered random variables. Thus, we can use Bernstein's inequality (cf. Theorem 2.10 \cite{boucheron2013concentration}) to obtain a concentration bound. To this end, we first see that 
$$ Y_{ij}^l = \begin{cases}1 &\text{ with probability }p^2\frac{w^*_l}{(w^*_l+z^*_i)(w_l+z^*_j)} \\ 0 &\text{ with probability } 1-p^2\frac{w^*_l}{(w^*_l+z^*_i)(w_l+z^*_j)}   \end{cases}\,, $$

$$ \E[{Y_{ij}^l}^2] = \frac{p^2w^*_l}{(w^*_l+z^*_i)(w_l+z^*_j)}\,. $$
We can now apply Bernstein's inequality to obtain
\begin{equation*}
\begin{aligned}
\Pr( \lvert P_{ij} - P^*_{ij}\rvert > t) &= \Pr\bigg( \big\lvert \sum_{l=1}^n Y^{l}_{ij} - \E[Y_{ij}^{l}] \big\rvert > td\bigg)\\
&\leq 2\exp{-\frac{t^2d^2}{ 2\bigg(\sum_{l=1}^n \frac{p^2w^*_l}{(w^*_l+z^*_i)(w_l+z^*_j)} +  \frac{td}{3} \bigg) }}\,.
\end{aligned}
\end{equation*}
This completes the proof.
\end{proof}

We have the following useful results which provide bounds on the total variation distance distance as well as the $\ell_2$ error of the stationary distribution of a Markov Chain from a \emph{reference reversible Markov Chain}:

~\\
\textbf{a. Total variation perturbation bound for reversible Markov Chains}
\begin{lemma}\label{lem:total-variation-bound-mc} (Theorem 2 of \cite{agarwal2018accelerated}, originally due to \cite{mitrophanov2005sensitivity}) Consider two discrete time Markov Chain $P$ and $P^*$ with finite state space and stationary distribution $\pi$ and $\pi^*$, respectively. If there exists a positive constants $R > 1$ and $\rho < 1$ such that:
$$ \lVert P^t(x, \cdot) - \pi^* \rVert_{TV} \leq R\rho^t, t = 1, 2,\ldots $$
then we have:
$$ \lVert \pi - \pi^* \rVert_{TV} \lesssim \lVert P - P^* \rVert_{\infty} $$
\end{lemma}

~\\
\textbf{b. $\ell_2$ perturbation bound for reversible Markov Chains}
\begin{lemma} (Lemma 2 of \cite{negahban2017rank}) Consider the setting of lemma \ref{lem:total-variation-bound-mc}, then:
$$ \frac{\lVert \pi - \pi^* \rVert}{\lVert \pi^*\rVert} \lesssim \lVert P - P^* \rVert_{2} $$
\end{lemma}

\begin{lemma} (Lemma 8 of \cite{chen2019spectral}) Consider the setting of lemma \ref{lem:total-variation-bound-mc}, then:
$$ \lVert \pi - \pi^* \rVert_{\pi^*} \leq \frac{\lVert {\pi^*}^\top(P^* - P)\rVert_{\pi^*}  }{\mu(P^*) - \lVert P - P^* \rVert_{\pi^*} } $$
where $\mu(P^*)$ is the spectral gap of $P^*$.
\end{lemma}

~\\
\subsection{A first analysis attempt}

One difficulty of the analysis of the Rasch model compared to the analysis of the BTL model is the dependence between the pairwise estimate $P_{ij}$ and $P_{kj}$. As a first analysis attempt, we will provide a concentration bound on the individual entry error $\lvert P_{ij} - P^*_{ij}\rvert$ and rely on union bound to provide a bound on $\lVert P - P^* \rVert_{\infty}$. We have the following result which bounds the entrywise error $\lvert P_{ij} - P^*_{ij}\rvert$.
\begin{lemma}\label{lem:error-concentration-bound-large-d} (Large self-loop)  If we set $d = mnp$, then
$$ \Pr(\lVert P - P^* \rVert_{\infty} > t ) \lesssim \sum_{i=1}^m \sum_{j\neq i }\exp{-\frac{t^2np }{ p\kappa + t }} $$
for some constant $\kappa$ to be determined.
\end{lemma}

\begin{proof}
\begin{equation*}
\begin{aligned}
\Pr(\lvert P_{i\cdot} - P_{i\cdot}^*\rvert > t) &= \Pr(\lvert \sum_{j=1}^m P_{ij} - P^*_{ij} \rvert > t )\\
&= \Pr(\lvert \sum_{j\neq i} P_{ij} - P^*_{ij} \rvert > t/2 )\\
&\leq \sum_{j\neq i} \Pr(\lvert P_{ij} - P^*_{ij}\rvert > \frac{t}{2(m-1)})\\
&\lesssim \sum_{j\neq i} 2\exp{-\frac{t^2d^2}{ 8m^2\bigg(\sum_{l=1}^n \frac{p^2w^*_l}{(w^*_l+z^*_i)(w_l+z^*_j)} +  \frac{td}{6m} \bigg) }}
\end{aligned}
\end{equation*}
Suppose that for all $l\in [n]$ and $i, j\in [m]$, $\frac{p^2w^*_l}{(w^*_l+z^*_i)(w_l+z^*_j)} \leq \kappa$ for some constant $\kappa$ to be determined. We have:

\begin{equation*}
\begin{aligned}
\Pr(\lvert P_{i\cdot} - P_{i\cdot}^*\rvert > t) &\lesssim \sum_{j\neq i} \exp{-\frac{t^2d^2}{ 8m^2\bigg(\sum_{l=1}^n \frac{p^2w^*_l}{(w^*_l+z^*_i)(w_l+z^*_j)} +  \frac{td}{6m} \bigg) }}\\
&\lesssim \sum_{j\neq i} \exp{-\frac{t^2d^2}{ m^2\bigg(np^2\kappa +  \frac{td}{m} \bigg) }}\\
&\asymp \sum_{j\neq i} \exp{-\frac{t^2d^2}{ m^2np^2\kappa +  mtd  }} \\
&\text{Substituting $d\asymp mnp$ gives}\\
&\asymp  \sum_{j\neq i} \exp{-\frac{t^2m^2n^2p^2 }{ m^2np^2\kappa +  tm^2np }} \\
&\lesssim \sum_{j\neq i} \exp{-\frac{t^2np }{ p\kappa + t }}
\end{aligned}
\end{equation*}
\end{proof}

\begin{lemma}\label{lem:error-concentration-bound-small-d}  (Small self-loop) If we set $d \asymp mnp^2$, then
$$ \Pr(\lVert P - P^* \rVert_{\infty} > t ) \lesssim \sum_{i=1}^m \sum_{j\neq i }\exp{-\frac{t^2np^2 }{ p\kappa + t }} $$
for some constant $\kappa$ to be determined.
\end{lemma}

\begin{proof} 
The proof is almost identical to that of lemma (\ref{lem:error-concentration-bound-large-d})
\begin{equation*}
\begin{aligned}
\Pr(\lvert P_{i\cdot} - P_{i\cdot}^*\rvert > t) &\lesssim \sum_{j\neq i} \exp{-\frac{t^2d^2}{ 8m^2\bigg(\sum_{l=1}^n \frac{p^2w^*_l}{(w^*_l+z^*_i)(w_l+z^*_j)} +  \frac{td}{6m} \bigg) }}\\
&\lesssim \sum_{j\neq i} \exp{-\frac{t^2d^2}{ m^2\bigg(np^2\kappa +  \frac{td}{m} \bigg) }}\\
&\asymp \sum_{j\neq i} \exp{-\frac{t^2d^2}{ m^2np^2\kappa +  mtd  }} \\
&\text{Substituting $d\asymp mnp^2$ gives}\\
&\asymp  \sum_{j\neq i} \exp{-\frac{t^2m^2n^2p^4 }{ m^2np^2\kappa +  tm^2np^2 }} \\
&\lesssim \sum_{j\neq i} \exp{-\frac{t^2np^2 }{ \kappa + t }}
\end{aligned}
\end{equation*}
\end{proof}

~\\
\textbf{Large self-loop construction with $d=mnp$}
~\\
An immediate consequence of lemma (\ref{lem:error-concentration-bound-large-d}) is that by setting $t = \frac{1}{\sqrt{\log m}}$ and so long as we have sufficiently large number of students (compared to the number of tests) such that:
$$ p \kappa = \frac{\log m}{n} \lesssim \frac{1}{\sqrt{\log m}} \Leftrightarrow  n \gtrsim (\poly\log m)\,, $$
Then $p\kappa \lesssim t$. The exponential concentration bound simplifies to 
$$ \Pr(\lVert P - P^* \rVert_{\infty} > t ) \lesssim \sum_{i=1}^m \sum_{j\neq i }\exp{-\frac{t^2np }{ t }} \lesssim \sum_{i=1}^m \sum_{j\neq i }\exp{-tnp } \,.$$
$$ \Pr(\lVert P - P^* \rVert_{\infty} > \frac{1}{\sqrt{\log m}} ) \lesssim \sum_{i=1}^m \sum_{j\neq i }\exp{-\frac{np}{\sqrt{\log m}} } \,.$$
~\\
So long as $np \gtrsim \poly\log m$, we have $\lVert P - P^* \rVert_{\infty} \lesssim \frac{1}{\sqrt{\log m}}$ with probability $1 - O(\poly(m))$. \emph{If the spectral gap} of the Markov Chain $P^*$ can be bounded below by a constant, then:
$$ \lVert z - z^* \rVert_1 \lesssim \lVert P - P^* \rVert_{\infty} \lesssim \frac{1}{\sqrt{\log m}} $$

~\\
Additionally, using the fact that $\lVert P - P^* \rVert_{op} \leq \sqrt{\lVert P - P^*\rVert_1 \cdot \lVert P - P^* \rVert_{\infty} }$ and the fact that both $\lVert P - P^*\rVert_1$ and $\lVert P - P^* \rVert_{\infty}$ can be bounded in the same way, we also have 
$$ \frac{\lVert \pi - \pi^* \rVert_2}{\lVert \pi^* \rVert_2} \lesssim \frac{1}{\sqrt{\log m}} $$
with probability $1 - O(\poly(m))$ so long as $ np \gtrsim \poly\log m $ and that the spectral gap of the Markov Chain $P^*$ can be bounded below by a constant.

~\\
\duc{If the spectral gap scales as $\frac{mnp^2}{d} = p$ then we will be in trouble. Experimentally, when $d=mnp$, the constructed Markov Chain seems to have terrible mixing time (slow convergence). }

~\\
\duc{If $m=n$ and $p \asymp \frac{\log n}{n}$, the probability with which a problem is not selected by any students is as $1-(1-\frac{\log n}{n})^n \geq 1- \exp{-\log n} = 1- \frac{1}{n}$}

~\\
\textbf{Small self-loop construction with $d=mnp^2$}

An immediate consequence of lemma (\ref{lem:error-concentration-bound-small-d}) is that by setting $t = \frac{1}{\sqrt{\log m}}$, the exponential concentration bound simplifies to 
$$ \Pr(\lVert P - P^* \rVert_{\infty} > \frac{1}{\sqrt{\log m}} ) \lesssim \sum_{i=1}^m \sum_{j\neq i }\exp{-\frac{t^2np^2}{\kappa} } \,.$$
~\\
So long as $np^2 \gtrsim \poly\log m$, and \emph{if the spectral gap} of the Markov Chain $P^*$ can be bounded below by a constant, then:
$$ \lVert z - z^* \rVert_1 \lesssim \lVert P - P^* \rVert_{\infty} \lesssim \frac{1}{\sqrt{\log m}} $$

~\\
Similarly, we have:
$$ \frac{\lVert \pi - \pi^* \rVert_2}{\lVert \pi^* \rVert_2} \lesssim \frac{1}{\sqrt{\log m}} $$
with probability $1 - O(\poly(m))$ so long as $ np^2 \gtrsim \poly\log m $ and that the spectral gap of the Markov Chain $P^*$ can be bounded below by a constant.

~\\
\textbf{Some preliminary experiment results.} Consider the following experiment: Let there be $n$ students and $m$ tests. $w^*_l = 1$ for all $l \in [n]$ and $z^*_m$ has been generated as a uniform grid from $0.05$ to $2$ (i.e., \verb|np.linspace|). We set $m = n$ and vary both quantities and measure how $\frac{\lVert \pi - \pi^* \rVert_2}{\lVert \pi^* \rVert_2}$ depends on the problem parameters and the sampling regime.

\begin{figure}[H]
\begin{centering}
    \begin{subfigure}{1.\textwidth}
    \centering
    \includegraphics[scale=0.45]{pics/dense.png}
    \caption{Performance of the spectral estimator (averaged over 50 trials), sparse sampling regime $p=4\log m/n$. Intuitively, the spectral algorithm should be able to do well in the sparsest sampling regime. However, these experiment results say otherwise.}
    \end{subfigure}\\
    \begin{subfigure}{1.\textwidth}
    \centering
    \includegraphics[scale=0.45]{pics/sparse.png}
    \caption{Performance of the spectral estimator (averaged over 50 trials), dense sampling regime $p=\sqrt{\log m/n}$. We already have the theory to back up this dense sampling regime.}
    \end{subfigure}
  \end{centering}
  \label{fig:performance-sparse-dense}
\end{figure}

==> analysis/topology_dependent_upper_bound.tex <==
\textbf{Topology}

In practice, we may not be given a randomly designed assignment graph

Suppose that we are given a fixed assignment $A$.

\duc{Implications in practice: bad examples of assignment vs good assignment}

\duc{Show that the accelerated spectral method produces the same stationary distribution as the vanilla spectral estimator}

==> problem_setup/problem_setup.tex <==
\section{Problem setup}\label{sect:problem-setup}
Suppose that in a final exam, there are $n$ students and $m$ total problems. Each student has a latent ability parameter $w_l > 0$ for $l = 1, \ldots, n$. Each problem has a latent difficulty parameter $z_i>0$ for $i = 1,\ldots, m$. If student $l$ is given problem $i$, she can solve the problem correctly with probability $\frac{w^*_l}{w^*_l + z^*_i}$. Let $X_{li}$ be the random indicator variable for the event that student $l$ solves problem $i$. For each student $l$, let $\calP_l$ be the set of problems assigned to her. We assume that the student attempts all of the problems assigned to her. Per the Rasch model, we assume that $\{X_{li}\}_{i\in \calP_l}$ are independent binary random variables. For two problems $i, j$, let $\Ss_{ij}$ denote the set of students who were assigned both problems. 
